Cost Models for Big Data Query Processing: Learning, Retrofitting, and Our Findings

Query processing over big data is ubiquitous in modern clouds, where the system takes care of picking both the physical query execution plans and the resources needed to run those plans, using a cost-based query optimizer. A good cost model, therefore, is akin to better resource efficiency and lower operational costs. Unfortunately, the production workloads at Microsoft show that costs are very complex to model for big data systems. In this work, we investigate two key questions: (i) can we learn accurate cost models for big data systems, and (ii) can we integrate the learned models within the query optimizer. To answer these, we make three core contributions. First, we exploit workload patterns to learn a large number of individual cost models and combine them to achieve high accuracy and coverage over a long period. Second, we propose extensions to Cascades framework to pick optimal resources, i.e, number of containers, during query planning. And third, we integrate the learned cost models within the Cascade-style query optimizer of SCOPE at Microsoft. We evaluate the resulting system, Cleo, in a production environment using both production and TPC-H workloads. Our results show that the learned cost models are 2 to 3 orders of magnitude more accurate, and 20X more correlated with the actual runtimes, with a large majority (70%) of the plan changes leading to substantial improvements in latency as well as resource usage.

==> cover-shep.tex <==
%!TEX root = main.tex

\section{Summary of Changes}

We thank the reviewers, the meta-reviewer, and the chairs for taking time to shepherd our paper.
Following the shepherding instructions, we ran additional experiments and gathered details that can be summarized as follows:

\begin{packed_enum}
\item Detailed explanation of the nature of SCOPE workload, showing the changes in a recurring job using a real example.
\item Re-training results over much larger workload and indicating how the workload is diverse in different business units, different job sizes, and even partially ad-hoc. 
\item Micro-experiments over a sample of training dataset to show why cardinality is insufficient for big data workloads.
\end{packed_enum}

For each of the shepherding instructions in {\color{red} red} below, we break down the part (12) of reviewer 1's comments into sub-comments (labeled R1.C1, R1.C2, and so on) in {\textbf{bold}} and highlight our proposed changes in {\color{blue} blue}.
%Our goal is to ensure that we are not misunderstanding any of the comments and that we are addressing the concerns to shepherd's satisfaction. 
We will be happy to further revise our changes based on recommendations from the shepherd.


\subsection{Shepherding Instruction 1}
\noindent\textcolor{red}{\it Clarify the nature of the workload and what happens to both learning and performance if the workload will be more diverse.}

\rcom{R1.C1}{Concretely, it would be great to learn more about the nature of the workload. The authors write that it consists of 850 recurring jobs in a 50K job/day workload (i.e. avg repeat of 60x per job).}

SCOPE workloads primarily consist of {\bf recurring jobs}. 
A recurring job in SCOPE is used to provide periodic (e.g., hourly, six-hourly, daily, etc.)  analytical result for a specific application functionality. Typically, a recurring job consists of a script template that accepts different input parameters similar to SQL modules. Each {\it instance} of the recurring job runs on different input data, parameters and have potentially different statements. As a result, each instance is different in terms of input/output sizes, query execution plan, total compute hour, end-to-end latency, etc.

To illustrate, Figure~\ref{fig:recurring_job_example_c} shows $150$ instances of an hourly recurring job that extracts facts from a production clickstream.
Over these $150$ instances, we can see a big change in the total input size and the total execution time, shown in blue and purples lines respectively.
Specifically, the input size varies from $69,859$ GiB to $118,625$ GiB, while the execution time varies from $40$ mins and $50$ seconds to $2$ hours and $21$ minutes.
%Here we provide one day history of an example recurring job in Scope which provides error and exception report for XBOX. For 24 instances of this hourly recurring job, we can see a big change in total data read, PN hour (total compute hour) and latency which indicates some changes in partitioning/sorting or physical operators in the execution plan. 
Therefore, a recurring job is {\it not} the same job repeating multiple times.
In fact, different instances of a recurring job can have very different query execution plans 
including different partitioning, sorting, physical operators, etc.


\begin{figure}
	\centerline {
		\hbox{\resizebox{\columnwidth}{!}{\includegraphics{shepherd/RecurringJobExample.pdf}}}}
	\vspace{-10pt}
	\caption{$150$ instances of an hourly {\it recurring job} that extracts facts from a production clickstream. }
	\label{fig:recurring_job_example_c}
	\vspace{-5pt}
\end{figure}


SCOPE workloads do contain a small portion of ad-hoc jobs as well. Figure~\ref{fig:non_recurring_jobs}, shows the percentage of ad-hoc jobs on four of the production clusters over three consecutive days. We can see that the percentage of ad-hoc jobs varies from $7\%-20\%$ on different clusters, and it also changes over days.
However, compared to ad-hoc jobs, recurring jobs represent long term business logic with critical value, and hence the primary focus for performance improvement in this paper.

\begin{figure}
	\centerline {
		\hbox{\resizebox{0.9\columnwidth}{!}{\includegraphics{shepherd/workload_nonrecurring.pdf}}}}
		\vspace{-10pt}
	\caption{Illustrating ad-hoc jobs in SCOPE. }
	\label{fig:non_recurring_jobs}
		\vspace{-5pt}
\end{figure}




\hide{
\stitle{What are recurring jobs?} A recurring job refers to one or more jobs that perform similar business tasks. For example, Figure~\ref{fig:recurring_job_example} shows instances of hourly and daily jobs for extracting facts from production click-streams, all collectively referred as a single recurring job. Notable aspects of recurring jobs include:
\begin{packed_enum}

\item Two instances of a recurring job typically have varying parameters (e.g., for extracting different facts), inputs (e.g., clickstreams arriving every hour), and the number of machines (depending on inputs / task) allocated to them. Indeed, we can see in Figure~\ref{fig:recurring_job_example}, the input size as well as the execution time for the recurring job can vary over a wide range. Finally, recurring jobs can also have varying logical plans (e.g., job instances analyzing daily clickstream vs hourly cickstreams) Thus, \emph{a recurring job is not the same job repeating multiple times. Further, it is rare to see the exactly same job running multiple times with the same input and same parameters.}

\item Because of the above reasons, recurring jobs can have different physical plans over different instances. For example, a recurring job involving the same $5$ logical operators, with each logical operator having $3$ possible physical operators, there can be as many as $ 3^5 = 243$ physical plans. In addition, if we also consider dynamic allocation of resources, the space of possible plans is even larger.
\end{packed_enum}
}

\pchange{
\begin{packed_enum}
 \item We define and clarify the nature of recurring jobs by summarizing  the above mentioned points in Section~\ref{sec:recurring}, in particular that a recurring job can behave differently over different instances.
 \item We explain that our workload consists of $7\%-20\%$ ad-hoc jobs on a daily basis (Section~\ref{sec:recurring} and Section~\ref{sec:experiments}~(See Workload)).
\end{packed_enum}}

\hide{
\begin{table}
	%	\begin{center}
	\caption{\rev{Nature of workload}}
	\label{tab:metadatanew}
	\vspace{-12.5pt}
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{ p{4cm}|l|l|l|l  } 
			\hline
			Metric (per day) & Cluster 1 & Cluster 2 & Cluster 3 & Cluster 4\\ \hline
			Total Jobs & 65113 & 44394 & 16401 & 29967 \\ \hline
			Recurring Jobs  & 52740 (80\%) & 36136 (81\%) & 13625 (83\%) & 25306 (85\%) \\ \hline
			Recurring Templates  & 17662 & 6044 & 2696 & 5917\\ \hline
			Avg. Daily Job Variation  & 8\%  & 20\% & 12\% & 2\%\\ \hline
			Total Sub-Expressions & 3284706 & 2232402 & 1326588 & 536294 \\ \hline
			%			Repeated Sub-Expressions & 2633981 & 1624081  & 1023611 & 408397 \\ \hline
			Recurring Sub-Expressions & 468643  & 522783 & 235668 & 53819 \\ \hline
			Ad-hoc Expressions & 182082 & 85538 & 67309 & 57698 \\ \hline
		\end{tabular}%
	}
	%	\end{center}
	\vspace{-10pt}
\end{table}
}


\begin{figure}
%	\vspace{-39pt}
	\centerline {
		\hbox{\resizebox{\columnwidth}{!}{\includegraphics{shepherd/workload_summary.pdf}}}}
	\vspace{-10pt}
	\caption{Considering a bigger workload of close to $0.5$ million jobs from $4$ production clusters over $3$ days.}
	\label{fig:workload_summary_c}
	\vspace{-15pt}
\end{figure}


\begin{figure*}
	\vspace{-30pt}
	\centerline {
		\hbox{\resizebox{\textwidth}{!}{\includegraphics{shepherd/workload_changes.pdf}}}}
		\vspace{-5pt}
	\caption{Illustrating workload changes over different clusters and different days. }
	\label{fig:workload_changes}
		\vspace{-10pt}
\end{figure*}

\rcom{R1.C2}{Show that either the workload is highly diverse and queries do not repeat or  rerun all the main experiments on a workload that is highly diverse and where jobs do not repeat (abstracting from certain job parameters that will obviously be different)}, and

\rcom{R1.C3}{It is also not known what happens to both learning and performance if the workload would not have this limited diversity and high repetition count.}

We now consider a much larger workload trace from $4$ different production clusters comprising of $423$ virtual clusters, with each virtual cluster roughly representing a business unit within Microsoft, and consisting a total of $\approx 0.5$~million jobs over $3$ days, that ran with a total processing time of $\approx 6$~million hours, and using a total of $\approx 1.4$~billion containers. 
Figure~\ref{fig:workload_summary_c} summarizes this larger workload. 
\hide{As depicted in Figure~\ref{fig:workload_summary}, our workload roughly consists of 80\% recurring jobs and fairly substantial 20\% ad-hoc jobs. Moreover, we felt it is important to clarify that recurring jobs are not repeating jobs.}


\stitle{Diversity.} \hide{As mentioned in the previous comment, our workload indeed does consists of about 20\% ad-hoc jobs. Moreover, we found the workload pattern to be similar across four different clusters, which shows that the pattern is common.}
We found the above larger workload to exhibit the following variety.
First of all, the workload is from $423$ different virtual clusters, each roughly mapping to a business unit, with very different set of applications that are expressed as SCOPE scripts.
Second, the workload on different clusters varies not just in terms of the load (e.g., more than $3 \times$ jobs on Cluster1 compared to Cluster4), but also in term of job properties such as average number of operators per job ($50s$ in Cluster1 compared to $30s$ in Cluster4) and the average total processing time\footnote{Total processing time of a job is the sum of processing time of all the containers used in that job.} per job (around $17$ hours in Cluster1 compared to around $5$ hours in Cluster4).
Third, the workload changes from day1 to day2 and then again from day2 to day3. Figure~\ref{fig:workload_changes} shows these daily changes on the four clusters. 
We can see that the changes could vary from a $30\%$ decrease to a $20\%$ increase on different clusters and different days.
And finally, the workload consists a mix of both recurring and ad-hoc jobs, with Figure~\ref{fig:non_recurring_jobs} showing $7\%-20\%$ ad-hoc jobs on different clusters and different days.

Note that even though our workloads have the above variations, we do not claim our techniques will be applicable to completely ad-hoc workloads. We are happy to clarify this better in the paper.


\stitle{Learning.}
We retrained all of our models on the above larger workload. In addition to showing the accuracy of learned models on all jobs, we now isolated the accuracy results of ad-hoc jobs. Specifically, Figure~\ref{fig:overallaccuracyresults} and Figure~\ref{fig:nonrecurringaccuracyresults} show the CDF of estimated vs actual costs. 
We can see that the charts resemble the ones shown in the paper, and are consistent across all clusters.
%of the learned models. 
Table~\ref{tab:medianaccuracy} summarizes the median accuracy of the combined model on each of the four clusters, and compares it with the default cost model.
%on median accuracy for the default cost model and the combined learned model for each of the cluster.
Table~\ref{tab:cluster1results} further breaks down the accuracy results on Cluster1
%show a more detailed breakdown on all and ad hoc jobs on cluster 1 
in terms of Pearson correlation, median error, 95\%tile error, and the model coverage, for both overall and ad-hoc jobs.

Interestingly, \emph{the accuracy and Pearson correlation over ad-hoc jobs drop slightly but it is still close to those over all jobs (Table~\ref{tab:cluster1results_c} and Table~\ref{tab:medianaccuracy_c})}. This is because: (i) ad-hoc jobs can still have one or more similar subexpressions as other jobs (e.g., they might be scanning and filtering the same input before doing completely new aggregates), which helps them to leverage the subgraph models learned from other jobs. This can be seen in  Table~\ref{tab:cluster1results} --- the sub-graph learned models still have substantial coverage of subexpression on ad-hoc jobs. For example, the coverage of $64\%$ for Op-Subgraph Approx model means that $64\%$ of the sub-expressions on ad-hoc jobs had matching Op-Subgraph Approx learned model. (ii)  Both the operator and the combined models are learned on a per-operator basis, and have much lower error ($42\%$ and $29\%$) than the default model ($182\%$). This is because the query processor, the operator implementations, etc. still remain the same, and their behavior gets captured in the learned cost models. Thus, even if there is no matching sub-expression in ad-hoc jobs, the operator and the combined models still result in better prediction accuracy. 



\eat{We retrained all of our models on the above larger workload.
Figure~\ref{fig:overallaccuracyresults} shows the model accuracy on different clusters. We can see that the results resemble the ones shown in the paper.
\hide{Besides, as mentioned in the previous comment, recurring jobs further abstract job parameters, input data, number of machines, and even vary logical operators. Indeed, as reviewer 1 mentioned, abstracting parameters is a typical way to vary characteristics of workload, and recurring jobs naturally model this.}
We further isolated the accuracy results of ad-hoc jobs in Figure~\ref{fig:nonrecurringaccuracyresults}. Interestingly, we see the accuracy to be SOME NUMBERS. 
This is because ad-hoc jobs can still have one or more similar subexpressions as other jobs (e.g., they might be scanning and filtering the same input before doing completely new aggregates), which helps them to leverage the subgraph models from other jobs. Furthermore, both the operator and the combined models are on per-operator basis, and so even if the job is ad-hoc, the cluster environment, the query processor, the operator implementations, etc. still remain the same, and their behavior gets captured in the learned cost models.
}

\hide{
\emph{Key point on Operator-model.} Operator models, like default cost models, learn a cost model for each operator (ignoring subplans), and thus they can used for  predicting costs on any arbitrary unseen plan. As can be seen in Figure~\ref{fig:overallaccuracyresults} and Figures~\ref{fig:nonrecurringaccuracyresults} and also across multiple experiments in the paper, the accuracy of operator-model is much better than default models, and thus even if specialized subgraph models completely, CLEO gives more accuracy than the default cost model.
}


\begin{figure*}
	\vspace{-40pt}
	\hspace{-0.1cm}
	\centerline {
	\hbox{\resizebox{\textwidth}{!}{\includegraphics{figs/overall_accuracy.pdf}}}}
	  \vspace{-25pt}
	\caption{Accuracy results on all jobs (recurring + ad-hoc) over four different clusters.}
	\vspace{-5pt}
	\label{fig:overallaccuracyresults}	
\end{figure*} 

\begin{figure*}
	\hspace{-0.12cm}
	\centerline {
		\hbox{\resizebox{\textwidth}{!}{\includegraphics{figs/nonrecurr_accuracy.pdf}}}}
	\vspace{-25pt}
	\caption{Accuracy results on only ad-hoc jobs over four different clusters.}
	\vspace{-5pt}
	\label{fig:nonrecurringaccuracyresults}	
\end{figure*} 


\begin{table*}
	\small
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{l|c|c|c|c|c|c|c|c} 
			\hline
		     & \multicolumn{4}{c|}{\textbf{All jobs}}  & \multicolumn{4}{c}{\textbf{Ad-hoc jobs}} \\ \hline 
			& Correlation &  Median Error &  95\%tile Error & Coverage &
			Correlation &  Median Error &  95\%tile Error & Coverage \\ \hline 
			\textbf{Default}  & \textbf{0.12} & \textbf{182\%} & 12512\% & \textbf{100\%}
			& \textbf{0.09} & \textbf{204\%} & 17791\% & \textbf{100\%}  \\ \hline
			Op-Subgraph  & 0.86 & 9\% & 56\% & 65\% 
			& 0.81 & 14\% & 57\% & 36\% 		\\ \hline
			Op-Subgraph Approx & 0.85  & 12 \% & 71\%& 82\% 
			&  0.80  & 16 \% & 79\% & 64\% 	 \\ \hline
			Op-Input & 0.81 & 23\% & 90\% & 91\%
			& 0.77 & 26\% & 103\% & 79\% 		 \\ \hline		
			Operator & \textbf{0.76} & 33\% & 138\% & \textbf{100\%} &
			\textbf{0.73} & \textbf{42\%}& 186\% & \textbf{100\%} 
			\\ \hline
			\textbf{Combined} &  \textbf{0.79} & \textbf{21\%} & 112\%  & \textbf{100\%} 
			& \textbf{0.73} & \textbf{29\%} & 134\% & \textbf{100\%}
			\\  \hline
		\end{tabular}%
	}
	%	\vspace{-2pt}
	\captionof{table}{\small Breakdown of accuracy and coverage of each learned model for all jobs and ad-hoc jobs separately on Cluster1.}
	\label{tab:cluster1results_c}
	\vspace{-20pt}
\end{table*}

\begin{table}
	\small
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{l|c|c|c} 
			\hline
			Cluster & Default (all jobs) & Learned (all jobs) & Learned (ad-hoc jobs) \\ \hline 
			Cluster 1 & 182\% & 21\% & 29\%\\ \hline
		   Cluster 2  & 256\% & 33\% & 40\% \\ \hline
			Cluster 3 & 165\% & 26\% & 38\% \\ \hline
			Cluster 4 & 153\% & 15\% & 26\% \\ \hline
		\end{tabular}%
	}
	%	\vspace{-2pt}
	\captionof{table}{\small Median accuracy of default and combined learned model over all jobs and ad-hoc jobs on each cluster.}
	\label{tab:medianaccuracy_c}
	\vspace{-25pt}
\end{table}



\stitle{Performance.} 
Given that re-training on the above larger workload does not change our conclusions on the learning accuracy, the same applies for performance.
This is because we chose a sample of jobs that had plan changes, due to better cost estimates from learned models, for our performance experiments.
Unless the cost model accuracies are different, the plan changes will remain the same and hence our selection of jobs for performance experiments.

\hide{As we mention in Section 6.5.1, for our performance experiments, we considered only 845 jobs, i.e., each recurring job once. Thus, the 845 jobs are ad-hoc (different) with respect to each other. Among them, we selected a subset for jobs with changed plans after training and feedback. We also present a case-study on a general TPC-H benchmark, explaining in detail the plan changes caused by the learned cost models. We, therefore, feel it is better to avoid further experiments on performance, which is difficult to do in a short timeline. Further, modifying (e.g., runtime) and using production resources is costly.}

\pchange{
\begin{packed_enum}
\item We describe workload details (Figure~\ref{fig:workload_summary}) from $4$ different production clusters  in Section~\ref{sec:experiments} (See Workload).
%, explaining clearly that our workload consists of $20\%$ non-recurring jobs on a daily basis.
\item We show retraining results for learned models for each of the four clusters, consisting of both recurring and ad-hoc jobs. We also separately show the prediction results on only ad-hoc jobs (up to $20\%$ of daily jobs)  (Table~\ref{tab:medianaccuracy}, Table~\ref{tab:cluster1results}).
\item Due to space constraints, we show the CDF distribution of prediction accuracy for each of the learned models for all jobs as well as for only ad-hoc jobs in our technical report~\cite{techreport}. Figure~\ref{fig:overallaccuracyresults} and Figure~\ref{fig:nonrecurringaccuracyresults} in the cover are depicted as Figure 12 and Figure 13 in technical report. Similarly, we show the CDF distribution of prediction results for different machine learning algorithms in Figure 9 in our technical report. Nevertheless, we show the overall results, i.e., median accuracy and and the Pearson correlation results, for each of the ML algorithms in Sections 3 and 4 in the paper.
\end{packed_enum}
}
\hide{\pchange{Comparing the accuracy of operator model and default model, we will explain why learned models do better than default models even for arbitrary new jobs consisting of unseen subplans.}}






	
\rcom{R1.C4}{Cynically one may say it is a decision problem in identifying one out of 850 plans given a query.}	

\noindent
Our learning problem is different from a  ``decision problem of identifying one out of 850 plans'', because 
%of the following reasons. 
as explained in response to R1.C1, each instance of a recurring job can have a very different query execution plan.
Furthermore, we predict operator level costs that are combined to pick the overall plans and with more accurate costs the optimizer can pick plans that have not been seen before.
%\begin{packed_enum}
%\item Depending on input characteristics, parameters, number of machines, as well as logical operators, the same recurring job can have different plans for different instances. Thus, as illustrated in our response to R1.C1, each recurring job in practice can have as many physical plans there can be combinations of physical operators for the logical operators in the job.
%
%\item CLEO's learned models predict the cost of each physical operator that are combined together, in the same way as existing optimzer, to get the overall plan. Thus, we do not directly predict the overall plan given a job, which we believe is quite challenging, and currently very difficult to do using machine learning techniques.
%
%\item  Combining the operator-wise or subplan-wise predictions can result in completely new overall plan. Thus, the generated plan may not be even present in training dataset. 
%	
%\end{packed_enum}
Finally, note that $835$ was just a small workload subset shown earlier. 
Overall workloads are much larger and we now show results on close to $100K$ recurring templates, and additional ad-hoc jobs.


\pchange{We add more details in Section~\ref{trainfeedbak} to explain how costs are predicted and combined, and that they can result in an arbitrary unseen plan. We also explain in 
Section~\ref{sec:tradeoff} how operator models can be used for predicting any unseen plan and that they have better accuracy than default cost models.}


\rcom{R1.C5}{And maybe these 850 jobs are also similar among them? There is no information in the paper, and this does matter a lot.}	

We measure the similarity of jobs using number of common sub-expressions, recurring sub-expressions, and ad-hoc sub-expressions, as shown in Figure~\ref{fig:workload_summary}.
% (we call them subgraphs in the paper). More is the number of subplans matching, the more similar are the set of jobs. 
Furthermore, each subgraph (i.e, Op-subgraph, Op-subgraphApprox, Op-input)  model learns at different granularity of sub-expressions, and therefore the coverage of these models indicates the similarity of jobs. For instance, in Figure 13a, the coverage of Op-Subgraph models (the strictest possible matching) is 39\% after 14 days, from which we can infer that jobs on day 14 had 39\% similar sub-expressions (ignoring parameters and inputs) to those on day 1. 
\hide{
Similarly, we provide statistics for each subplan coverage / \% on our workload in Table 7. Also, please see our point on Operator-model that describe why CLEO results in more accuracy even when jobs are dissimilar.
}

\pchange{
We explain more explicitly how we can infer similarity of jobs using coverage of models in Section~\ref{sec:accuracy} (see only ad hoc jobs).}


\hide{
\stitle{General Remarks.} If it helps, we are happy to clarify in the paper that our work focuses on workloads with high percentages of recurring jobs, and that fully exploring the capabilities of CLEO on extremely ad-hoc workloads is a future work. Nevertheless, as can be noticed from the nature of workloads from four different clusters, the workload patterns that CLEO exploits are  ubiquitous. 
}

%Additionally, we now provide extra details in a x-page technical report that we were unable to fit in the paper due to page limits. That said, the paper by itself is self-sufficient, and readers may not need to refer to the technical report to understand the core ideas and empirical results presented in the paper.

\vspace{-5pt}
\subsection{Shepherding Instruction 2}
\noindent\textcolor{red}{\it Back up the statement on why perfect cardinality estimation is quite inadequate for query optimization in a distributed setting.}


%\stitle{M4. More details on why perfect cardinality is inadequate.} 

\rcom{R1.C6}{The authors also stay by their statement that perfect cardinality estimation is quite insufficient for doing query optimization in a distributed system.	This statement is interesting, as it goes counter to what has been believed so far, and reported on recently.We do not see detailed insights (backed by experiments) on how this can be explained.}

\hide{
Cost models combine statistics such as (e.g., cardinality, average row length, selectivity) by assigning them weights to predict the cost of operators. We observed two key issues that result is less accuracy of predicted costs despite using perfect cardinality estimates. First, traditional cost models use a very small number of statistics to model a cost. Second, the weights assigned to statistics are typically fixed and remain same across all workloads and systems. Further, the weights are bench-marked or updated once in many years since it is tedious to update them frequently. We conducted two micro-experiments to highlight the resulting issues.
}

To backup our claims on cardinality, we ran the following two micro-experiments over a sample of $200$K sub-expressions from the Cluster4 workload shown in Figure~\ref{fig:workload_summary_c}.

\begin{figure}
	\centerline {
		\hbox{\resizebox{1.1\columnwidth}{!}{\includegraphics{figs/featureVsErrors.pdf}}}}
	\vspace{-12pt}
	\caption{Impact on median error as we cumulatively add features from left to right. The first two features are perfect output (C) and input (I) cardinalities.}
	\vspace{-15pt}
	\label{fig:cumfeatureErrorc}
\end{figure}


\vspace{0.1cm}
\noindent\textbf{Micro-experiment 1: need for more features.}
Starting with perfect cardinality estimates (both input and output) as only features, we fitted an elastic net model to find / tune the best weights that lead to minimum cost estimation error (using the loss function described in Section~\ref{sec:learningmodel}). Then, we incrementally added more and more features while also combining them polynomially with previously selected features, retraining the model with every addition. Ultimately, we end up with the same set of features as used in the paper. 

Figure~\ref{fig:cumfeatureErrorc} shows the decrease in cost model error as we cumulatively add features from left to right.
The notations for features depicted on the X axis are defined in Table~\ref{tab:basicfeatures} and Table\ref{tab:derivedfeatures}.
We make the following observations.
\begin{packed_enum}

\item When using the perfect cardinalities, the median error is about $110\%$. However, when adding more features, we observe that the error drops by more than half to about $40\%$.
This is because of the more complex environments and queries in big data processing that are very hard to cost with just the cardinalities (as also discussed in Section 2.3). 
%SCOPE workloads, for instance, see widespread use of UDFs that are very difficult to cost with just cardinality.

\item Deriving additional statistics by transforming (e.g., sqrt, log, squares) input and output cardinalities along with other features helps in reducing the error. However, it is hard to arrive at these transformations in hand coded cost models.

\item We also see that features such as parameter (PM), input (IN), and partitions (P) are quite important, leading to sharp drops in error. While partition count is good indicator of degree of parallelism (DOP) and hence the runtime of job; unfortunately query optimizers typically use a fixed partition count for estimating cost as discussed in Section 5.2. 

\item Finally, there is a pervasive use of unstructured data (with schema imposed at runtime) as well as custom user code (e.g., UDFs) that embed arbitrary application logic in big data applications.
It is hard to come up with generic heuristics, using just the cardinality, that effectively model the runtime behavior of all possible inputs and UDFs.

\end{packed_enum}

\hide{
\emph{The need for more features:} Figure~\ref{fig:cumfeatureError} shows the decrease in error of cost model as we cumulatively add features from left to right. We do not show the features that did not reduce the error. The notations for features depicted on the X axis are defined in Table~\ref{tab:basicfeatures} and Table\ref{tab:derivedfeatures}. The left-most $4$ or $5$ features are frequently used statistics in traditional cost models. We see that if we only use input and output cardinality (both perfect), the median error is about 110\%. On adding more features on the right, we observe that the error can be reduced by more than half to about 40\%. However, cost models typically do not use that many statistics. In addition, we also see that deriving additional statistics by combining functions (e.g., sqrt, log, squares) of input and output cardinalities with other features helps in reducing the error.
}

%Using features based on parameter (PM) and input template names help directly learn the runtime behaviour of queries from past execution traces.

\vspace{2pt}
\textbf{Micro-experiment 2: varying optimal weights.} We now compare the optimal weights of features of physical operators when they occur in different kinds of sub-expressions. 
We consider the popular hash join operator and identified two sets of sub-expressions in the same sample dataset:
(i)~hash join appears on top of two scan operators, and 
(ii)~hash join appears on top of two other join operators, which in turn read from two scan operators each.

\hide{We present an example of HashJoin physical operator. Using a subset of jobs from cluster 4, we created two workloads based on the following patterns. In workload 1, HashJoin occured on top of two Scan operators, and in workload 2, HashJoin is at the root of two other join operators, which in turn read from two Scan operators each. 
For simplicity, we focus on top $10$ features that lead to minimum error of HashJoin on both workloads.}


\eat{
\begin{figure}
	\vspace{-39pt}
	\centerline {
		\hbox{\resizebox{1.05\columnwidth}{!}{\includegraphics{figs/featuredifferences.pdf}}}}
	\vspace{-12pt}
	\caption{Hash join operator having different weights over different sub-expression sets.}
	\vspace{-12pt}
	\label{fig:differrentweights}
\end{figure}
}


Figure~\ref{fig:differrentweights} shows the weights of the top $10$ features of the hash join cost model for the two sets.
%over workload 1 and workload 2 for HashJoin operator. 
We see that the  partition count is more influential for set 2 compared to set 1. This is because there is more network transfer of data in set 2 than in set 1 because of two extra  joins. Setting the partition count that leads to minimum network transfer is therefore important. On the other hand, for jobs in set 1, we notice that hash join typically sets the partition count to the same value as that of inputs, since that minimizes repartitioning. Thus, partition count is less important in set 1. 
To summarize, even when cardinality is present as a raw or derived feature, its relative importance is instance specific (heavily influenced by the partitioning and the number of machines) and hard to capture in a static cost model.
%Similarly, we observed that weights of statistics can vary across clusters, and even on the same cluster depending on number of machines. 

%However, default cost models typically use the same fixed weights for all instances of the same operator.

\pchange{We added two micro-experiments in Section~\ref{sec:cardLearner} reporting and briefly summarizing the above analysis.} 
\hide{We think a more thorough study of the interplay between cardinality and cost models in distributed settings is a good avenue for future research.}





	
%\stitle{B. Impact of Cardinality Estimation}

%Please see our response to M4.

\rcom{R1.C7}{Personally, my doubt is whether the failure of query optimization in the face of perfect cardinality estimation could still not be explained by optimizer shortcomings.}

We highlighted two key reasons why cost models suffer with poor accuracy despite feeding in perfect cardinality estimation.
SCOPE has been a topic of active research and although it has been the backbone for analytics workloads at Microsoft for the last decade, it still has its own shortcomings.


\pchange{ 
We added references to the large body of prior work on SCOPE to give more context in Section~\ref{sec:scopebackgnd}.
}
% on the things that have been tried and results reported in the previous studies.
%
%We will add more reference 
%We will further add references to a large body of prior work on SCOPE, given that SCOPE has been in production for more than a decade running one of the largest analytical workloads in industry 
%
%  and will explain that the SCOPE optimizer is not new --- it has been in existence and has been manually tuned over years to efficiently support a large number of users and jobs on a daily basis. It would be difficult to operate at such a massive scale with a naive optimizer.
% 


\subsection{Changes for space}
In order to make space, we have moved the following content to our technical report~\cite{techreport}.
\shep{
\begin{packed_enum}
\item Cross-Validation results. We have moved experiments on cross-validation results on different machine learning models to Section 6.1 in technical report. Nevertheless, we report the median accuracy and pearson correlation results for each ML model in Section 3 to 4 in the paper.
\item CDF of accuracy results for the four clusters.  In our technical report, we show the CDF distrbution of prediction accuracy for each of the learned models for all jobs as well as for only ad-hoc jobs. (Figure~\ref{fig:overallaccuracyresults} and Figure~\ref{fig:nonrecurringaccuracyresults} depicted as Figure 12 and Figure 13 in technical report).
\item We have moved the figure showing feature weights for  op-subgraph-Approx, op-subgraph-input and operator models as Figure 5 in the technical report. 
\item In addition, due to space constraints, we show  Figure~\ref{fig:non_recurring_jobs} and Figure~\ref{fig:workload_changes} depicted earlier in this cover in our technical report as Figure 3 and Figure 10, and describe the changes in workload and ad hoc jobs in text in Section~\ref{sec:recurring} and Section~\ref{sec:experiments} in the paper. The changes can also be inferred from Table 7 in the paper.
\end{packed_enum}
}




==> cover.tex <==
%!TEX root = main.tex

\section{Summary of Changes}


%\vspace{2cm}
We thank the reviewers and the meta-reviewer for their insightful
and detailed feedback,
and for giving us a chance to address their comments. 
%We believe that our paper has immensely benefited from their feedback.
Below, we first describe how we addressed the meta-reviewer comments and provide a summary of the changes made to the paper.
Next, we respond to the common comments raised in the reviews.
And finally, we respond to each of the individual comments from the reviewers.
All changes to the paper are highlighted in {\color{blue} blue}, and are also referred to in  {\color{blue} blue} in our response below.
%Additionally, we now provide extra details in a x-page technical report that we were unable to fit in the paper due to page limits. That said, the paper by itself is self-sufficient, and readers may not need to refer to the technical report to understand the core ideas and empirical results presented in the paper.

%\subsection*{Meta-reviewer Comments}
\rcom{M1}{Why this is specific to serverless query processing}.

\noindent\rev{We have replaced serverless with ``big data systems'' throughout the paper, including in the title.} 
%\rev{We have also changed the title of the paper from} ``Cost Models for Servlerless Query Processing: Learning, Retrofitting, and Our Findings'' to \rev{``Cost Models for \textbf{Big Data} Query Processing: Learning, Retrofitting, and Our Findings''}. 
\rev{In Section~\ref{sec:related} (Related Work), we now clarify how our work is related  and applicable to serverless systems, along with relevant references.}

\rcom{M2}{Comparison to an additional piece of related work.}

\noindent\rev{We now compare with CardLearner~\cite{cardLearner} both empirically (Section~\ref{sec:cardLearner} and Figure~\ref{fig:cardlearner}) as well as qualitatively (Section~\ref{sec:cardLearner}) in terms of accuracy of cost estimates, problem addressed, coverage, as well as techniques used.}

%Here, we assume that the meta-reviewer is referring to CardLearner, as also mentioned by R4. Please see our response  to 3. 

\rcom{M3}{More details on various aspects of work.} 

\noindent We added all of the details requested by the reviewers throughout the paper, including:
\begin{packed_enum}
\item[1.]  \textit{Workload Metadata and Generalizability} (R1).\rev{We now provide more details on workload metadata and each of the learned models in our experiments in Section~\ref{sec:experiments} (see Table~\ref{tab:metadata}). We also report the training time and other overheads in more detail in Section~\ref{sec:overhead}. We further explain how our key idea of using common sub-expressions is typical in other enterprise settings in Section~\ref{sec:learningmodel}}.

\item[2.] \textit{Instrumentation and scaling to large number of models} (R4).\rev{ We rewrote the earlier section~\ref{trainfeedbak} to provide more details on instrumentation and how we scale to large number of sub-graphs. In addition, we also added more experiments in Section~\ref{sec:overhead} where we describe the overhead of instrumentation and using learned models for cost-prediction per job. We also show training time for one of the clusters consisting of more than $800$ unique recurring jobs, with tens of thousands of jobs instances in total.}


\item[3.] \textit{ Efficiency of resource exploration (R3).}
\rev{We conducted additional experiments to provide more details on efficiency-accuracy trade-off of resource exploration. In particular, we replaced the older Section 6.3 on accuracy of partition exploration with a new accuracy-efficiency trade-off on partitions.} 

\item[4.] \textit{ Justification on loss function (R3).}
\rev{We now describe why we choose the specific loss function better, and show a micro-benchmark that reports the 5-fold cross-validation results of commonly used regression-based loss functions.}
\end{packed_enum}

%Please see our response to 2,4,5,6.
\vspace{1cm}
\rcom{Other changes}{}

\noindent 1. {\it Presentation, typos, and size of figure and tables.}
\rev{We thank the reviewers for spotting these. We have fixed all typos, grammatical errors, and presentation issues throughout the paper, to the best of our abilities. 
We have also increased the size of figures and tables throughout the paper.}

\noindent 2. {\it Changes for space.}
In order to make space, \rev{we have moved the section on Discussion to Section 6.6 in our technical report~\cite{techreport}. In addition, we also moved the figure for cross validation results of operator-sub-graphApprox model to the technical report.} The  operator-sub-graphApprox has similar results to that of operator-input model in Figure~\ref{fig:ml_cv}.



%\vspace{10pt}
\section{Common Comments}

\rcom{C1}{Serverless query processing (R1, R3, R4).}

\noindent By ``serverless'', we meant all cloud-based big data systems where an optimizer picks both the execution plan as well as the resources required to run a query. One widely accepted definition of ``serverless'' is that \emph{it is a cloud computing execution model where the cloud provider dynamically manages the allocation and provisioning of servers''}~\cite{serverless}. Similarly, in \scope{}, users do not need to worry about
cluster allocation nor do they manage any infrastructure; rather,  users pay only for the queries that they run. In fact, \scope{} is not much different from
Athena~\cite{aws-athena} and ADLA~\cite{adla}, which are considered serverless as per their web-pages~\cite{aws-athena,azurewebpage}. \rev{In Section~\ref{sec:related} (Related Work), we now clarify this and explain how our work is related  and applicable to serverless systems, along with relevant references.} Since \system integrates resource optimization within the query optimization itself, we believed \system is more useful to serverless relative to other systems where resources, e.g., number of machines, are pre-defined. 

That said, we agree with reviewers that our ideas are useful and can be generalized to all big data systems. We also agree that focusing on serverless may lead to misunderstanding and limit the applicability of our work.
%Therefore, we made the following additional changes. 
\rev{Therefore, we have replaced serverless with ``big data systems'' throughout the paper, including the title.} 
%\rev{We have also changed the title of the paper from} ``Cost Models for Servlerless Query Processing: Learning, Retrofitting, and Our Findings'' to \rev{``Cost Models for \textbf{Big Data} Query Processing: Learning, Retrofitting, and Our Findings''}.
%Unlike a typical cluster environment,  CompanyY's infrastructure is a sizable private cloud that runs massive volumes and variety of workloads, and shares typical characteristics of


\rcom{C2}{Comparison with CardLearner~\cite{cardLearner} (earlier [33]) (R4).}

%\rev{We now compare with CardLearner~\cite{cardLearner} both empirically (Section~\ref{sec:cardLearner} and Figure~\ref{fig:cardlearner}) as well as qualitatively (Section~\ref{sec:cardLearner}).}  
\noindent The key differences can be summarized as follows.
\begin{packed_enum}
	\item \textbf{Problem addressed}. \system predicts \emph{cost} while CardLearner predicts \emph{cardinality}. Cardinality is one of the features that cost depends on. Thus, CardLearner cannot be used for predicting cost for selecting optimal physical plans. In fact, as we note in Figure~\ref{fig:costModelwithCardFeedback}, even an hypothetical ideal cardinality estimation approach cannot lead to accurate cost prediction. Thus, there is a strong need for accurately modeling the query costs in big data systems, which is what we address in this work. \rev{We now make this point more clear in Section~\ref{sec:intro} and Section~\ref{sec:motivation}, citing CardLearner as well as additional cardinality models~\cite{stillger2001leo,cardLearner,lightweightCardModels,corrJoinsCardModels}.}
	
	\item \textbf{Empirical comparison}. \rev{In Section~\ref{sec:cardLearner}, we compared the accuracy of costs when using CardLearner, with both \system as well as the default cost model}. Our results shows a wide gap in the median error ($211$\% for CardLearner with default cost model versus $18\%$ for \system) as well as Pearson correlation ($0.01$ for CardLearner with default cost model versus $0.80$ for \system) when we compare the cost-estimates with the actual runtimes on production workload. These results are consistent with our discussion in Section~\ref{sec:intro} and Section~\ref{sec:motivation} where we argue that even ideal cardinalities may not be sufficient to fix the cost modeling in big data systems.
	
	\item \textbf{Novel techniques in \system for achieving full coverage with high accuracy}. CardLearner only learns models for recurring sub-graphs, similar to operator-subgraph models in \system, and therefore has a partial coverage (up to 55\%). Thus, in a given plan, if the CardLearner model doesn't exist for an operator, CardLearner uses default cardinality models. Unfortunately, using two disparate models for predicting cost in the same plan can lead to errors as costs are combined across operators and therefore need to be in the same scale (as also mentioned by Reviewer 1 in comment D4 on LEO). Thus, for any cost modeling approach to be useful, it \emph{must} provide  full (100\%) coverage. Therefore, \emph{achieving full coverage with high accuracy} is one of the core challenges that we address in our work.  \system learns four different types of sub-graphs models and combines them using an ensemble, which we believe are very different from CardLearner, and novel for cost estimation in query optimizer.
%	novel ideas from query optimization perspective, and are very different from CardLearner work.  
\rev{We now make this point more clear in Section~\ref{sec:related}}.
	
	\item \textbf{Resource Exploration and Cascades Integration}. Given that resources, such as number of machines, is an important factor for cost-estimation in big data systems, \system uses an efficient exploration algorithm to pick both query and resource optimal plans. Moreover, \system extends Cascades framework for effective integration of learned models. Resource exploration was not a subject matter in CardLearner. \rev{We also make this point more clear in Section~\ref{sec:related}}.
	
\end{packed_enum}

\rcom{C3}{Generalizability (R1).}

\begin{packed_enum}
%\item \textbf{Workload Metadata}. \rev{We now provide more details on workload metadata, including the numbers on each learned models along with additional characteristics in Section~\ref{sec:experiments}: Table~\ref{tab:metadata}. We also report the training time and other overheads in more detail in Section~\ref{sec:overhead}.}
	
\item \textbf{System and workload.} \textbf{A)} \system exploits common subexpressions in SystemX production workloads to learn specialized models. These patterns are also typical in other enterprise settings, e.g., three VLDB'19 papers (SparkCruise, Helix, Alibaba). \rev{We now explain this in more detail in  Section~\ref{sec:learningmodel}}. \textbf{B)}  Besides specialized models, our ideas on combining models using an ensemble and  adding resource-awareness are generalizable to other query engines such as Spark and are not specific to \scope{} workloads. \textbf{C)}  Our optimizer integration and Cascades framework extensions for making it resource-aware are not specific to \system. Variants of Cascades frameworks are used in systems like SQL Server, Spark, Calcite, etc. and hence they can also benefit from our proposals. \rev{We, now,  make this point clear in Section~\ref{sec:resourceopt}.} \textbf{D)} We also present results on TPC-H benchmark, in addition to production to show the effectiveness of our proposed solution on more general benchmarks.

\item \textbf{Overfitting.}
It is worth noting that the training sample size is small mostly for the individual models, especially the operator-subgraph and the operator-subgraphApprox models as they are more specialized. For these models, \system uses elastic net, instead of trees or neural networks. Elastic net, a $L_1$ and $L_2$ regulaized linear regression model, is relatively less prone to overfitting as we explain in detail in  Section~\ref{sec:learningmodel}. We use FastTree regression algorithm only for the combined model. Since there is only one combined model for each operator, the training sample size is much larger (orders of $1000$). Moreover, the features to combined model include predictions from individual elastic net models that further help minimize overfitting. 
Indeed, our $5$-fold cross validation results depict that the FastTree regression results in better accuracy compared to neural network. 
This is consistent with findings from other recent works that also find trees performing a little better than NNs over their workloads~\cite{lightweightCardModels, cardLearner}.

With regards to generalizability of machine learning models used in \system, we would like to emphasize that none of our core ideas are tied to machine learning models used. Specifically, the training features, the three specialized sub-graph structures that help mitigate the accuracy-coverage gap, the idea of combining models using an ensemble for robustness, the optimizer integration, and the Cascades extension for resource-exploration, can all work seamlessly with any machine learning model. In fact, we explored five different
machine learning models in the paper. Depending on the workload characteristics, the selection of final model can vary. All our results are based on 5-fold cross validation(CV)  on production workloads. Thus, one can similarly use CV to decide the most suitable model. 
%\todo{We should also respond to the comment that "tree-based models are just enormous overfits anyway"} \tar{Done.}

\item \textbf{How representative is \scope{}.} We want to highlight that SystemX has been the analytics backbone of CompanyY for more than a decade, \rev{serving a very wide mix of business units}, and there are many prior works that describe its optimizer (evolved over many years) as well as the diversity and generalizability of its workloads. \rev{At several places in the paper, we have now provided relevant metadata on this. In addition, we will also be able to refer the readers to prior work on \scope{} and its workloads after the double-blind process is over.}
\end{packed_enum}
	
\hide{
\rcom{R3}{Query plan instrumentation, and scaling to large number of sub-plan models.}

\rev{We rewrote the earlier section 6.4 to provide more details on instrumentation and how we scale to large number of sub-graphs. In addition, we also added more experiments in Section 6.3 where we describe the overhead of instrumentation and using learned models for cost-prediction per job. We also show training time for one of the largest cluster consisting of more than 1000 unique recurring jobs, with tens of thousands of jobs instances in total.
}

\rcom{R2}{Efficiency of resource exploration.}

\rev{We conducted additional experiments to provide more details on efficiency-accuracy trade-off of resource exploration. In particular, we replaced the older Section 6.3 on accuracy of partition exploration with a new accuracy-efficiency trade-off on resources.} In summary, ...
	
	

\rcom{R2}{Justification on loss function.}

\rev{We now better describe why we choose the specific loss function, in addition to providing a micro-benchmark that reports the 5-fold cross-validation results of commonly used regression-based loss functions.} In summary, ...
}



%\vspace{20pt}



\section{Reviewer 1}

\rcom{R1.W1}{Overfitting. It is unclear how well the proposed solutions could hold up for others who try to use it. Neural networks do not work well, due to few training samples; and therefore overfitting -- and my fear here is that the tree-based models are just enormous overfits anyway. The problem is that the authors do not disclose enough information about their workloads Also, the quality of the proposed solution (the ensemble model) for CompanyY may be fine but in case CompanyY has a very repetitive workload any algorithm that memoizes (just: caching) would do fine. Likely this solution does not work at all well for other use cases.}
TODO.

\noindent Please refer to C3 above for a discussion on generalizability of our approach and how we have addressed that in the revision. 
The reviewer also raised an interesting point about caching which merits some discussion below. We have not included this in the paper since discussion on caching was not explicitly asked for the revision, however, we will be happy to include it in the final version if desirable.

%Three points:\\
%
%\noindent 1. {\it Caching.} Indeed many of the business critical production workloads are repetitive. Some examples could include web index builder, pipelines for advertiser feedback loop, relevance/ranking algorithms, analyzing user experience from the telemetry, and gathering recommendations for products.
%These application involve large scale data processing tasks that 
First of all, it is worth noting that repetitive queries are typically templatized with different parameters and inputs that change over time, e.g., daily, hourly, etc. 
%(exact same queries on the exact same inputs does not make sense anyways). 
As an example, consider a daily query that analyzes the previous week's data, processing, for instance, 100GB inputs on day 1 and 120GB inputs on day 2. Simply caching the costs from day 1 and reusing them on day 2 will lead to arbitrary errors, since the new input will have more partitions and hence very different costs. Likewise, many other parameters change over time as well. So just caching from past workload does not generalize to future workload even for CompanyY. The other problem with caching is that it can easily lead to very high storage and lookup costs, i.e., storing (and efficiently looking up) the costs from all sub-plans of all past queries in the cloud is non-trivial. A learned model can represent the same information in a much more compact (and resilient) manner. This argument is similar to those made in recent works on learned index structures~\cite{kraska2018case}: for a given dataset one could easily ``cache" the index positions of keys, which is what traditional indexes do anyways; a learned index, however, can do the same thing with a much smaller storage footprint and faster lookups.

\hide{
\noindent 2. {\it Generalizability.} As noted in the paper, there is a significant chunk of the workload that is not repetitive, i.e., we cannot build operator-subgraph models for that portion of the workload. 
Handling this non-repetitive part of the workload and making the learned cost models work more in general is in fact one of our major contributions in the paper (see Section 4). In contrast to operator-subgraph models that leverage workload overlaps, the other most general extreme would  be learn a model per operator. Our approach is to bridge these two extremes of generality and learn multiple models with varying degree of generality and then combine them into a single uber model.
Note that we are not suggesting a new cost model for commodity databases that would just work off the shelf for any workload. 
Instead, our argument is that we can extract patterns that are quite typical in production workloads and combine them to instance optimize the cost model for a given cloud workload. 
The four patterns we considered are:
(1) common subexpressions, which is a typical pattern reported in several enterprise workloads such as~cite{..}, (2) similar subexpressions, where we have used one notion of similarity, but one could easily extend to other notions of similarity as well, (3) subexpressions that operate on the same base inputs, since multiple queries are likely to process a given set of inputs in realistic workloads, and finally (4) considering only the operators which is the most general scenario anyways. 
We showed that these four patterns yield accurate and robust cost models on SystemX, but one could further incorporate other patterns that might be specific to other systems.\\

%We are trying to balance between specialization and generalization: it is very hard to build accurate cost models for commodity databases, so our approach is to consider large cloud workloads where we have previous performance logs. 

\noindent 3. {\it Ensemble.} The ensemble model is not linked to any specific system or workload pattern. The ensemble model simply says that if you have a set of different models with different levels of generality, combining them can generate a model that can have full coverage and yet good accuracy. We used 4 individuals in the paper but one could further think of more individual models, based on other interesting patterns they might see in their workloads, and add them into the ensemble. {\bf Tarique} -- may be you can say better why ensemble is not overfitting anyways ...
}


\rcom{R1.W2}{Presentation of tables and figures. 
\eat{The paper has squeezed too much space, and has effectively squeezed the tables and figures out of visibility for people beyond their thirties. The font sizes in tables 1-4 must be increased by a factor 1.5 at least.Figure 5 is a readability joke (we are supposed to see pixels there) and Figures 6-8 must also be increased by a factor 1.5-2 to become parsable to the himan eye. And yes, that means that you have to delete text.}}

\noindent We thank the reviewer for highlighting this. \rev{We have fixed this throughout the paper.}


\rcom{R1.W3}{Contributions. a) ... giving a recommendation for resource usage is something that parallel database systems have done forever -- they do so even under resource constraints, i.e. taking into account the concurrent query workload and try not to use more resources than available.}


\noindent Our main contribution is exploring resources \emph{within} the big data query optimizer. 
Unfortunately, the state of the art techniques in big data processing pick resources for a fixed physical query plan \emph{output by the optimizer}~\cite{jyothi2016morpheus,perforator}.
%In contrast, prior work estimate resources, outside the optimizer, for a fixed physical plan output by the optimizer.
Not exploring resources within the query optimizer leads to sub-optimal plans as also highlighted in prior work~\cite{raqo}.
\rev{We now explain the differences more clearly in Section~\ref{sec:related}.}

	
	
\rcom{R1.W3b}{Also, the use of data mining techniques as used here for query optimization is not new, e.g. [2]. Hence, the contributions are less deep than they appear at first, on second though.}

\noindent We agree that using data mining techniques for query optimization is not new by itself. However, our main contribution is learning models such that we achieve both high accuracy and high coverage at the same time. In particular, our ideas on learning specialized models that exploit three frequently occurring workload patterns besides the operator model, using a combined model to achieve robustness, integrating the learned cost-models within the query optimizer, and efficiently exploring resources as part of query processing 
significantly advance the state of big data query optimizers in a production setting.


%   has not been proposed before. In addition, optimizer integration and resource-awareness ...\\
%We could re-emphasize our two key questions --- We investigate two major questions in this paper: (1) could we learn accurate, yet {\it robust}, cost models for big data workloads that are much more prone to estimation errors, and (2) could we integrate the learned within the query optimizer and produce both query and resource optimal plans. ... we could focus on the integration part a bit here ..



\rcom{R1.D1a}{on page 1 you say that you fed in the exact cardinalities into your Cascades model and it did not improve much. From this you conclude that cardinality estimation does not matter for Big Data systems -- despite all the evidence counter to this in other database systems.In other words, the fact that the query optimizer produces bad plans even when fed with perfect oracle cardinalities, could also be due something being wrong with the way this optimizer actually plans queries (or.. costs them). What the JOB paper basically said is that equating cost to intermediate result sizes works pretty well. But maybe your optimizer does something really strange in terms of cost derivation from the estimates.}

\noindent Prior work~\cite{leis2015good, lohman2014query} argue that correcting cost modeling  is less important, instead estimating accurate cardinalities is sufficient. In contrast, our empirical findings show that accurate cardinality estimation is not \emph{sufficient} for predicting accurate costs for large scale big data systems.
In fact, even when we feed the ideal cardinality estimates, there is little correlation between the predicted costs and the actual runtime of the queries.
This is for a variety of complexities, including presence of unstructured data that are hard to collect statistics on, user defined functions that are tedious to be cost estimated, distributed query processing that introduces more moving parts that are very difficult to model, and the cloud variance that adds yet another level of unpredictability in performance.
%This is inline with R1's point that ``something wrong with the way this optimizer actually plans queries (or.. costs them)''. 
Therefore, in this work, we develop learning techniques for improving query plan costing by automatically combining many of these factors for a given cloud environment at hand, i.e., learning for a specific deployment. 
%While we may not be sure that our proposed solutions may be as effective in traditional database systems where prior work have shown that the cardinality estimation is the core problem, 
We believe that our solutions are applicable and can help improve the performance of massively parallel big data systems (e.g., calcite, spark, Alibaba's internal system etc.) which share characteristics of our system. Trying out these techniques on traditional databases and investigating the role of cardinality there will be a part of future work.

	
\rcom{R1.D1b}{We do not know what your system is, but .. hm.. relatively new large-scale database systems at big tech firms are also not exactly known for their superb optimizer architectures.} 

\noindent SystemX has been the analytics backbone of CompanyY for
more than a decade, with many prior works describing its optimizer (evolved over many years), and diversity and generalizability of its workloads. 
Even mature open source systems like Hive and Spark could loose up to 2x performance by not picking partitions as part of query optimization~\cite{raqo}.
\rev{At several places in the paper, we now provide the relevant metadata on this. In addition, we will also be able to refer the readers to prior work on \scope{} and its workloads after the double-blind process is over.}


\rcom{R1.D1c}{One thing that needs to be incorporated is a good model for choosing parallelism (i.e. the number of partitions).
Many things can go wrong and a deeper investigation would have been in order before just giving up on "real" operator based query optimization, and drawing the conclusion that cardinality estimation is useless/hopeless in Big Data systems ...}

\eat{
 We do not want to advocate that cardinality estimation or heuristic-based cost modeling are hopeless. Instead, we want to present learning-based cost modeling as another possible or additional alternative, that the database community should consider  in the time ahead. We believe our work plays a significant step in that direction. For example, as we discuss in Section x, there have been continuous efforts, for over decades, to improve the cost modeling in query optimizer. Inspite of this, as show in Figure X, there improvement in cost accuracy has been marginal. We do not claim that our learned models will always be better than any hand-crafted cost models, however our empirical results show that difference in accuracy and correlation are substantial. \\
}

\noindent We do not discard cardinality and in fact we use cardinality estimates as features in learned cost models. 
Also, instead of replacing the entire optimizer with a learned one, our approach is more piecemeal which can work with existing cardinality estimator, search strategy, and transformation rules.
We only make the surgical change of replacing the cost model with a more accurate one that is learned from past workloads, and use the same model for partition exploration as well.
Our proposed partition exploration preserves the operator based QO, while adding a resource context for optimizing partitions per-stage. 
Essentially, the real change is how the sub-plan costs are derived, both with and without partition exploration, as depicted in Figure~\ref{fig:resplan} and Figure~\ref{fig:resplan_example}.

As we discuss in Section~\ref{sec:motivation}, there has been continuous efforts, for over decades, to improve the cost modeling in query optimizer.
Our own internal teams have spent months manually fine tuning the cost models.
Still, as we show in Figure~\ref{fig:costModelwithCardFeedback}, the improvement in cost accuracy has been marginal. 
Therefore, we want to present learning-based cost modeling as an alternative that the database community should consider.
We do not claim that our learned models will always be better than any hand-crafted cost models, however our empirical results show that differences in accuracy and correlation are substantial for large and diverse workloads.




\rcom{R1.D2}{Given the sparse examples of queries in the query logs you use for training, the huge danger of overfitting looms. You seem not to be worried by it. If, it works for you, you're happy. Well, fair enough. But what does that mean for the reader of SIGMOD proceedings; will this also work for me?
Indeed, if my workload is highly repeptitive, then over-fitting does not matter so much. But, if that is requirement for your system to be useful, I think the readers would like to know.}


\noindent Please see our response to C3.2 above on how \system is less prone to overfitting. We discuss the key ideas that are generalizable across systems below.

\system leverages multiple sub-graphs model with increasing training data (i.e., coverage). The combined model, further, helps in selecting the ideal sub-graph and combines their scores depending on performance.
%\tar{need to add more points}
Still, note that we are not suggesting a new cost model for commodity databases that would just work off the shelf for any workload.
Instead, our message to the readers of SIGMOD proceedings would be that one can extract patterns that are quite typical in production workloads and combine them to instance optimize the cost model for the given cloud workload at hand. 
The four patterns that we considered are:
(1) common subexpressions, which is a typical pattern reported in several enterprise workloads as discussed in C1 earlier, (2) similar subexpressions, where we have used a notion of similarity, but one could easily extend it to other notions of similarity, (3) subexpressions that operate on the same base inputs, since multiple queries are likely to process a given set of inputs in realistic workloads, and finally (4) considering just the physical operators which is the most general scenario anyways. 
We showed that these four patterns yield accurate and robust cost models on SystemX, but one could further incorporate other patterns that might be specific to their systems.

\rev{To show how multiple models with varying degree of generality help, we have now added Table~\ref{tab:metadata} that shows the coverage of individuals models as $61\%$, $82\%$, $93\%$, and $100\%$ (note that their accuracy is in reverse order as shown in Table~\ref{tab:modelaccuracies} and the heat map of Figure~\ref{fig:cov_accuracy_heatmap}).}

%Can we show the avg. number of training examples and the number of features for different individual models? .. this will help argue that sparse examples are also very specialized, i.e., fewer features, while the more generalized models have more examples.\\
%
%Other arguments: it is true that there is a very large space of possible query plans, 
%but this is also why we have focussed on cloud workloads since with the new emerging cloud data services there is a central place of observing massive query logs from the same underlying infrastructure. This was previously not possible with on-premise databases where every customer could only see their private query logs.


\rcom{R1.D4}{One of the problems that the real LEO project at IBM hit was that remembering real query cost did not help much. Even though cardinality and even runtime info in that (matching) part of the query was perfect, the overall results did not improve. This was because LEO needed to combine estimates based on perfect knowledge with estimates based on a cost model. As a way to deal with this problem, the idea of entropy maximization proposed. A computationally expensive technique, that still blocks its widespread adoption.
The integration of CLEO in the cascades optimizer is bound to be hitting similar problems, since it will cost different subplans and combine the cost. What are your thoughts on the reliability of making such combinations? After all, during query optimization different sub-solutions are combined and the complete query plan is constructed incrementally, whereby these intermediate comparisons determine what solution is chosen. Even if it is possible in the end to re-cost the whole query with the ensemble model, then it is remains unknown if wrong combinations of estimates on the subplan level have led one away from the optimal query plan.}

We thank the reviewer for mentioning this point. Providing 100\% coverage for all possible sub-plans has been the core challenge that \system addresses. The reviewer is absolutely right that we cannot use two disparate models for predicting costs across operators in the sample query plan. This is because costs across operators are compared and combined to predict the overall cost, and two disparate models can have different scales. In other words, comparing costs from two models is analogous to comparing currencies of two countries on the same scale.
Thus, for \system to be useful it must provide 100\% coverage, with high accuracy. We address this by learning an ensemble model that combines predictions across individual models to predict the final cost. This ensemble model is applicable for all query subplans, i.e., it has $100\%$ coverage. As a result, with \system, the predicted costs are never mixed or compared with the estimated ones.

Internally, the ensemble model uses predictions from disparate individual models only as \emph{features}. Note that the features of any machine learning model can be on  different scales. Essentially, the ensemble model learns a new function that adjusts and combines the predictions such that the predicted value is close to the actual runtime. Using the currency example, the combined model internally learns how to adjust the scale of two currencies so their comparison is meaningful.
Finally, note that ensemble models are not comparing or combining costs across sub-solutions using different individual models. 
Once the exclusive costs for operators are predicted using the ensemble model, they are combined the same way as it's done in the default optimizer to derive the cost of a sub-plan (or sub-solution).


\eat{
Moreover, we do agree with the findings from the LEO project that remembering the real query cost is less effective. This is one main reason why we do not learn models for the exact sub-graphs. As we describe in Section~\ref{sec:learnedcosts}, the  operator-subgraph model in \system, which is the most strict possible model, uses parameters and inputs as features rather than fixing them. There are additional features as listed in Table~\ref{tab:basicfeatures} and Table~\ref{tab:derivedfeatures} that can vary across queries and over time. Thus, we learn a behaviour of operator given all these features, which makes \system capture the space of possible predictions more flexibly and effectively than stricter models. To provide additional robustness to estimates, \system learns multiple models at different granularity, which are together combined using an the ensemble-based combined model. The ensemble model is less prone to overfitting and can effectively characterize the space where each model performs well. \todo{Its good to point out robustness, but then question is more about what happens when you have to combine actuals/estimates at any point}

\textbf{B. Computationally Expensive.}  As we describe in Section~\ref{trainfeedbak}, even though there are large number of models, each of which needs to be trained, we can easily do so offline using \scope{} based parallel trainer. For example, as explained in Section~\ref{sec:overhead}, \system learns $25$k models in less than $45$ minutes. Moreover, the elastic net and FastTree regressions are lightweight, taking only $600$MB of space when all $25$k models are loaded simultaneously. Finally, the overhead of $5-10$\% (order of milliseconds) for look-up is marginal compared to over compilation and runtime. Thus, the integration of \system within \scope{} query optimizer does not come with prohibitively large overheads. \todo{This does not seem to relate to the reviewer comment on LEO above.}

\textbf{C. Combining sub-solutions.} Finally, in \system, we reuse the same search strategy and the way sub-solutions are combined or prune as it is done in the default optimizer. As explained in Section~\ref{sec:learningmodel}, \system only replaces the default cost model for predicting each operator's ``exclusive'' cost. Our focus in this project is to improve the accuracy of cost estimates for each operator, which is currently done using cost models, one for each operator. Once the exclusive costs are predicted, they are combined the same way as it's done in the default optimizer. We agree with the reviewer that wrong search or combination strategy may lead us to a sub-optimal plan. However, we believe improving the search strategy is an important but complementary problem, which we plan to explore in the future. 
\tar{maybe we can also say such a change would be much more invasive ... moreover, should we add a few lines in the related work to acknowledge / clarify this, which I guess the reviewer also wants.}
\todo{I dont think it is about changing how the costs are combined or just about finding sub-optimal, its more about that when we combine costs (some are predicted from past workload and some estimated) we could also be hit by the same problem as LEO.}
\\

\todo{Somehow I feel this response does not address the reviewer comment precisely; we are going a bit orthogonal here. The key question is that LEO suffered from the problem of combining (or even comparing) actuals and estimates, which are two very different things on very different scales, and whether we will hit the same problem. While on the surface we can say that the combined model has $100\%$ coverage so we will not have this problem. But the individual models on the ensemble will have this problem, e.g., consider two subgraphs to a join operator; if they have different number of individual models available in their ensemble then the accuracy of their costs will be different and hence combining them will have interesting effects. I am guessing that we will only suffer from variable errors but the values are always on the same scale since they are all coming from one or more learned models. May be this could be middle ground that we could acknowledge..}
}

%Of course, the ensemble may have different number of individual models at different points in the query plan ....... whats our argument for this?



\section{Reviewer 3}
\rcom{W1.D1.D2.D3}{The paper bills itself as a paper about serverless query processing, but it really just seems to be about distributed query processing. The "serverless" aspect is not justified (See D1-D3)....Notably, there are no references to any papers about serverless computing. The recently published Berkeley tech report includes numerous citations that could be relevant: Eric Jonas et al. 2019. Cloud Programming Simplified: A Berkeley View on Serverless Computing. Technical Report UCB/EECS-2019-3. EECS Department, University of California, Berkeley. ...
Although the partition exploration that CLEO uses to select the optimal number of partitions per operator will be important in a serverless environment, there are numerous other requirements ....
 The contributions of this paper are broader than just ``serverless'' systems, and should be useful for distributed database systems in general.}

\noindent Please see our response to C1.

\hide{
\com{b. Although the partition exploration that CLEO uses to select the optimal number of partitions per operator will be important in a serverless environment, there are numerous other requirements for a database to be considered "serverless". As described, SystemX appears to be far from a serverless system. CompanyY is certainly aware of the computing resources it is using, and several of the machine learning models used by CLEO rely on the fact that the workloads are internal to CompanyY and are using subsets of the same large dataset. Although an individual user may not be aware of the resources used by an individual query, this is no different than how existing distributed databases work.}

The reviewer is right that CompanyY is aware of the computing resources, however, given the fact that the infrastructure is a sizable private cloud worth hundreds of millions of
dollars and running massive volumes (and variety) of workloads, it is no longer a typical cluster environment. In these environments, systems like SystemX are too complex to model costs using heuristics, and hence the need for CLEO.


\com{c. The contributions of this paper are broader than just ``serverless'' systems, and should be useful for distributed database systems in general. I think the connection to serverless is interesting and is worth mentioning in the discussion section of the paper, but defining CLEO as purely applicable to serverless systems is unnecessarily limiting.}
We agree with reviewers that using the word ``serverless'' may lead to misunderstanding and limit its applicability, therefore \rev{we have replaced serverless with ``big data systems'' throughout the paper. We have also changed the title from ... to .... Moreover, we have added a paragraph in the related work to describe how our work relates to serverless processing work, citing all relevant work from the area.}
}

\rcom{W2.D4}{The choice of loss function is not well justified (See D4)...The loss function defined in 3.1.2 seems somewhat arbitrary, and is never compared with other possible loss functions. The text mentions a couple of reasons for using logarithms, but since the choice of a loss function is such an important decision, I would have liked to see more justification (perhaps with a micro-benchmark)}

\noindent\rev{We now describe in more detail why we choose the specific loss function, as well as report a micro-benchmark that compares the accuracy of commonly used regression-based loss functions on our production workload.} 
In summary, using the mean-squared log error as the loss function makes \system less prone to outliers or large differences in costs. This is because the loss function essentially optimizes the ratio or percentage difference between the predicted cost and actual runtime. Our benchmark results show that the loss functions based on differences or squared differences result in lower accuracy. Those functions are more sensitive to extremely large differences between actual and predicted costs, which can occur when the job's running time itself is long or even due to machine or network failures typical in big data system.
Additionally, the mean-squared log error helps penalize under-estimation more than over-estimation, which is more desirable. The under estimation can lead to under allocation of resources which is highly undesirable. Finally, the log transformation implicitly ensures that the predicted costs are always positive.

\rcom{D5}{The paper does never explicitly mentions which approach is used by CLEO, or how to navigate the tradeoff between efficiency and accuracy.}

\noindent\rev{We now show experiments in Section~\ref{subsec:partexplore} to analyze the accuracy and efficiency trade-off between sampling strategies and the analytical approach.} Our results show that the analytical approach is about $20$$\times$ more efficient than the sampling approach for achieving the same accuracy. \system uses the analytical approach as the default strategy for finding the optimal resource, that we now more clearly explain in Section~\ref{subsec:partexplore}. For the same reason, we use the analytical approach for finding the optimal resource for the production experiments in Section~\ref{sec:perf}.


\rcom{D6}{ It seems like the first two scenarios described for the "Analytical approach" in Section 5.3 are reversed. If the first term in the cost equation is negative but the second is positive, it seems that it would be better to limit the number of partitions.}

\noindent We thank the reviewer for pointing this. \rev{We have fixed it in our revision.}

\rcom{D7}{Figure 7 is not well explained. Some references in the text (e.g. to the number of training samples used) do not appear to be visible in the chart. Additionally, it's very difficult to tell which line in each chart corresponds to which ML algorithm. Finally, it's not clear which model is used in 7(f).}

\noindent\rev{We have now fixed this in our revision.} In Figure~\ref{fig:learnedmodelaccuracy} (earlier Figure 7(f)), we use the elastic net algorithm for individual models, and the FastTree regression algorithm for the combined model. \rev{We now provide a more detailed explanation in Section~\ref{sec:evalMLAccuracy}.}


\rcom{D8}{Section 6.4.1 describes how 17 jobs were selected for experimentation. How representative is this sample? Approximately what percentage of the entire production workload would see a change in the query plan by using CLEO instead of the default optimizer?}

\noindent\rev{We now provide the details on plan changes in Section~\ref{sec:perf}.} We saw  about (22\%) of the jobs had plan changes when partition exploration was turned off, while ($39$\%) had plan changes when we also applied partition exploration. We observe similar results over TPC-H queries, about 28\% of the queries had plan changes. 
Note that production resources are expensive and so it is not possible to use the entire workload for performance experiments. 
Therefore, we selected a small subset of the workload by considering
jobs that had at least one change in physical operator implementations, e.g, for aggregation (hash vs stream grouping), join (hash vs merge), addition or removal of grouping, sort or exchange operators. 
From this set, we selected a sample of $17$ unique recurring jobs that had varying end to end latency and total processing times, i.e., considering jobs of different sizes.
%These jobs are representative of jobs executed in \system with varying end to end latency and total processing times.
While these jobs constitute a good sample of the workload that is impacted (positively or negatively) by \system{}, it is hard to claim that this is a representation of the overall workload.
Generating representative workload from a large corpus is a very interesting problem in itself for future research.

\eat{
Among these jobs, 70\% (12 Jobs) had improvements in runtime when optimized using \system. Similarly, about 83\% ($5/6$) of the TPC-H queries had improvements. Interestingly,  \system was able to improve the end-to-end latency for $10$ out of $12$ jobs with less degree of parallelism (i.e., the number of partitions). For the cases  the performance degrades, we describe practical techniques to address these in our production setting in our technical report. \tar{currently the above description sounds a bit weak on representative point ...} \todo{we should highlight that the perf experiments are expensive since they require production runtime environments, and so we could only test with a small subset; all other experiments are over entire workload.}
}

\rcom{D9}{In section 6.5, the paper suggests that it may be useful to optimize a query twice -- both with and without CLEO -- and use the learned models to choose the plan with lower predicted latency. This seems a bit odd, since the CLEO plan was produced with the learned models and presumably should always have lower predicted latency. Is there any evidence that the default plan would ever be chosen?}

\noindent Yes, while rare there are scenarios when the default plan can be chosen when we  optimize the query twice. For efficient exploration, optimizers follow a greedy strategy when searching for plans, where the selection of downstream operators essentially depends on upstream operators that have already been selected in the plan. While using \system, it is possible that \scope{} may select an upstream operator that leads it to a completely different search path, thereby missing the plan that was selected by the default cost model.
By optimizing twice, we at least ensure that we compare the plan chosen by \system with the plan that system would have chosen otherwise. This can help in preventing potential regressions.

We use the learned models for predicting the accuracy of the two plans because our experimental results show that learned models are highly accurate (18\% median error and 0.84 Pearson correlation) in predicting the runtime of an operator. The is $2$ orders of magnitude more accurate and $20$ times more correlated than the default cost models. Hence, learned cost models are more suited to compare two plans. Note that, in the above scenario, if the optimizer had not skipped the default plan, learned models would have anyways selected it if was more efficient. Moreover, the idea of using a learned model to compare two given plans to prevent regressions have also been used in prior work~\cite{ding2019ai}.

\rev{Given that our ideas on avoiding regressions are preliminary, we have moved the discussion section on this to our technical report~\cite{techreport}. This also helped us make space for incorporating new changes.}

\rcom{D10}{There are numerous typos and grammatical mistakes throughout the paper. Please proofread.}

\noindent We thank the reviewer for pointing this.  We have fixed them throughout the paper.


\section{Reviewer 4}
\rcom{W2.D2}{Not clear why the technique is limited to serverless computing ... Please elaborate on why CLEO is limited to serverless computing. It seems to me that CLEO is equally applicable to, e.g., a Hive or Presto cluster.}

\noindent Please see our response to C1.

\rcom{W3.D1}{Very close to [33] but does not provide a good comparison to that paper. Please provide a thorough comparison to [33]. The problem being addressed by both papers is the same, and the solutions share many similarities.}

\noindent Please see our response to C2.


\rcom{D3}{ CLEO requires the query plan to be instrumented so that each operator is annotated with its actual output cardinality and execution cost. The paper should include some information about how this instrumentation is done, and the overhead of this instrumentation.}

\noindent\rev{We now provide details on instrumentation and discuss why it's not a problem in in Section~\ref{trainfeedbak}}. In summary, big data systems, such as \scope{}, are already instrumented to collect logs of query plan statistics and runtime traces.  For uniquely identifying each operator/subplan, query optimizers annotate each operator with a \emph{signature}~\cite{bruno2013continuous}. We extended the optimizer to  compute three more signatures, 	one for each individual sub-graph model and extract additional statistics (i.e., features) that were missing for \system. Since all signatures can be computed simultaneously in the same recursion and there are only $25-30$ features per operator, most of which were already extracted, the total overhead is minimal.

\rev{We also show additional experiments in Section~\ref{sec:overhead} to report per job overhead in optimization time for \scope{} while using \system.} As depicted in Figure~\ref{fig:overheadtime}, we see most of the jobs have $5$-$10$\% increase in the optimization time. This overhead includes instrumentation, logging, the model lookup time and any additional exploration due to plan change. Since the optimization time is often in orders of few hundreds of milliseconds, the overhead incurred here is negligible compared to the overall compilation time (orders of seconds) of jobs in big data systems as well as the gains we can see in the end-to-end latency (orders of 10s of minutes) (Figure~\ref{fig:prodlatency}). 



\rcom{D4}{ CLEO learns a cost model for each observed query sub-plan. If the workload is sufficiently diverse, then there can be too many sub-plans to process. The paper deals with one aspect of this problem, specifically that some sub-plans will not have enough training data. However, there are potentially other aspects of the problem. For example, there can be too many plans to store and process, making the memory consumption or processing overhead of CLEO too high? Can the number of similar sub-plans reduce the accuracy of CLEO? Please elaborate on whether there are problems with having too many observed sub-plans, beyond the problem of too little training data for infrequent sub-plans, beyond Section 6.4.3.}

\noindent We respond to the two questions separately.

\stitle{A) Overhead of too many subplans.} \rev{We now provide more fine-grained details on the workload metadata, the number of models created for each sub-graph model, as well as the training time and memory consumption when all models are loaded simultaneously in Table~\ref{tab:metadata}, Section~\ref{trainfeedbak} as well as Section~\ref{sec:overhead}.}

In summary, as we describe in Section~\ref{trainfeedbak}, models are trained and processed in parallel using \scope{} itself. For example, for a cluster running $845$ unique recurring jobs daily, \system trains about $25K$ learned models in less than $45$ minutes over a cluster of $200$ nodes. All models relevant for a cluster are loaded upfront by the optimizer, into a hash map, to avoid expensive lookup calls during query optimization. When loaded simultaneously, all $25K$ models together take about $600$ MB of memory, which is within an acceptable range given that cloud optimizers can host $100s$ of GBs of physical memory. Finally, as we discuss in D4 above, the overhead in optimization time is $5$-$10$\% (orders of $100$s millisecond) which is negligible compared to the compilation time (orders of seconds) and gains in latency (tens of minutes) for big data jobs.

\stitle{B) Can the number of similar sub-plans reduce the accuracy of CLEO?.} It depends on how \emph{strictly} we define two sub-plans to be similar.
If the reviewer meant that the notion of similarity is strict (e.g., like in operator-subgraph), the accuracy further improves as the number of subplans increases, because the higher number of sub-plans reduce the overfitting and affect of noise. We discuss this issue in detail in Section~\ref{sec:learningmodel}. Unfortunately, it is rare for strict models, in practice, to have a large number of instances. In our production workloads, more than 50\% of such model have less than $30$ subplan instances.

On the other hand, when the notion of similarity is not strict (e.g., operator, or operator-input models), the number of sub-plans covered under a single model naturally becomes large. However, the accuracy can degrade when the variety of sub-graph/sub-plan instances under the same model increases.
 That is why, the accuracy of operator-input or operator models is less than operator-subgraph instances. As we explain in Section~\ref{sec:learnedcosts} and Section~\ref{sec:robustness}, different subplans can have very different performance behavior and can vary drastically depending on interactions with underneath operators via pipelining, sharing of sorting and grouping properties. Therefore, modeling them using a single learned model leads to lower accuracy.

Thus, generally speaking, a large coverage of subplans within the same model leads to less accuracy because of the variety of subplans. Table~\ref{tab:modelaccuracies} depicts this trade-off. There are exceptions when models are more strictly defined. In such cases, extremely few samples leads to less accuracy due to overfitting and noise, and large number of samples improve the accuracy. We describe this phenomena in Section~\ref{sec:combined} using the heatmap in Figure~\ref{fig:cov_accuracy_heatmap}. In order to automatically navigate this trade-off and characterize the space where each model performs well, \system uses the combined model. As depicted in Table~\ref{tab:modelaccuracies} and Figure~\ref{fig:learnedmodelaccuracy}, the combined model is able to provide the best of both worlds, i.e., accuracy close to those of strict sub-graph models and high coverage ($100$\%) that of the operator model.


\rcom{D5}{ The tables and figures in the paper are too small and difficult to read. Please make them bigger.}

\noindent We thank the reviewer for mentioning this. \rev{We have fixed them throughout the paper.}

\rcom{D6}{ Please add a few words on how to interpret Figure 1 when you first introduce it. For example, it is a CDF and the ideal shape is a step function at $10^0$.}

\noindent We thank the reviewer for mentioning this. \rev{We now do so in Section~\ref{sec:intro}.}


\rcom{D7}{ In Section 2.2, please elaborate a bit more on the five phases of the Cascades framework to provide more context about how CLEO fits in with the optimizer.}

\noindent The integration of learned models only requires changes to the fifth task: the optimize input. \rev{We now mention this more clearly in Section~\ref{sec:optoverview} and explain how \system fits it in Cascade framework along with the changes to Optimize Input task in detail in Section~\ref{trainfeedbak}: Model lookup with the help of Figure~\ref{fig:resplan}.} Because  of the space limitations, we are afraid we could only provide limited details on the first four phases of Cascades framework, that help with plan exploration and application of transformation rules. However, we have referred the readers to the Cascades paper~\cite{cascades95} that explains the four phases in detail. We believe that not explaining the them in detail does not affect the comprehensibility of the paper. Nevertheless, if the reviewer still thinks otherwise, we will be happy to fix it in our camera-ready version.  



\rcom{D8}{ One can think of a very large number of ways of combining the features in Table 1 to produce derived features. Why does CLEO use the specific derived features in Table 2? Elastic net selects the informative features, but what is set of input features given to elastic net?}

\noindent \rev{We now explain why feature selection is needed and our process better in Section~\ref{sec:featuresel}}.


\rcom{D9}{ Sections 5.1 and 6.5 can be shortened to make room for the additions requested above.}


\rcom{D10}{ Some typos...}

\noindent We thank the reviewer for listing them. \rev{We have fixed most of the grammatical errors and typos.}




==> partition_prev.tex <==
%!TEX root = main.tex

%\section{Partition-Aware Query Planning}
\section{Resource Awareness}
\label{sec:resources}

Traditionally, cost models assume a fixed set of resources, e.g., a given machine or a given cluster. However, with large public clouds and on-demand resource allocation, this assumption does not hold anymore. In this section, we look at the dual problem of incorporating resources awareness in the cost model and exploring the right set of resources given a resource-aware cost model. For the ease of presentation, we restrict ourselves to partition count (interchangeably also referred to as the degree of parallelism) in the discussion below, however, our approach can be easily extended to a more general vector of resources.
\tar{clarify more on why we focus only on degree of parallelism.}

\subsection{Traditional Query Planning}

\begin{figure*}
	\centerline {
		\hbox{\resizebox{\textwidth}{!}{\includegraphics{figs/resourceopt.pdf}}}}
	\vspace{-2.5pt}
	\caption{Illustrating Resource-aware Query Planning in \system.}
	\vspace{-13.pt}
	\label{fig:resourceopt}
\end{figure*} 

%As depicted in \add{Figure XX} \todo{point to important features}, partition count is an important determining feature of the cost of an operator. Recall that 
Partition count is the number of partitions into which an input to an operator is split. Typically each machine has one partition, therefore partition count also corresponds to the degree of parallelism (DOP) of the operator. The volcano style top-down query optimization allows to incorporate partition count as a required property from the upstream operators.
In practice, for distributed query planning, the partition count is propagated from the previous data distribution boundaries.
SCOPE, for instance, identifies the partition count at the {\it stage} boundaries, where a stage is a set of operators without any re-partitioning.
The operators at the stage boundaries include extractor from un-partitioned data, range reader on already partitioned data, and shuffle operator to re-partitioned data, collectively referred to as boundary operators which either load or partition datasets. Boundary operators compute the partition count based on heuristics, such as data size and skew. Physical operators, above the boundary operator, in a stage  set their partition counts to the value chosen by the boundary operator. This is because all operators belonging to the same stage must have the same partition counts. To illustrate, we consider an example query and the corresponding query plan shown in Figures~\ref{fig:resourceopt}(a) and Figure~\ref{fig:resourceopt}(b). 
Figure~\ref{fig:resourceopt}(c) shows the two stages created with resource-agnostic query planning. 
Operators in the first stage pick the partition count from the extractor operator, while the operators in the second stage pick the partition count from the shuffle operator. 

% Issues with existing approach.
There are several issues with this approach. 
First, given that the partition counts could be different for different stages, the cost model needs to consider the partition count for more accurate predictions.
Figures~\ref{fig:peroperatorsubgraph}--\ref{fig:peroperator} already shows how the partition count is an important feature in determining the cost of an operator. Now the query planner needs to invoke the model with the partition count chosen for each operator (or stage). This is in contrast to {\it bubble costing}~\cite{yint2018bubble} that costs all queries for a given fixed partition count.
Second, the partition count chosen by the boundary operators may not be the optimal for all operators in a stage. This is challenging because we cannot independently pick the optimal partition count for each operator either, since that might introduce many more stage boundaries and increase the overall query cost.
Therefore, there is need for jointly finding the partition count of all operators in stage that leads to the overall lowest cost. 

Below we describe our resource-aware query planning that we have implemented in SCOPE, which is a volcano style top-down query planner. Then we show further optimizations to make the planning more efficient.

\eat{
First, ... ignoring the impact of partition count on the cost of operators above boundary operators ... another operator can have lower cost than the chosen for a different partition count....]
Second ... earlier work \tar{cite ICDE paper} suggest that costs of two physical operators can conflict depending on the machines (same as the number of partition counts) allocated to each operator.


We state the problem formally,
\begin{problem}
Problem here...
\end{problem}


\subsection{Resource-aware Cost Model}

TODO: describe the additional resource feature
}

\subsection{Resource-aware Query Planning}
%\subsection{Finding Optimal Partition Count}
\label{sec:resourceopt}

We present a two-phase approach for resource-aware query planning in a Volcano-style top down query optimizer.
%In order to address the above problem, we use a two phase approach.
The first phase is {\it partition exploration}, where each physical operator recursively passes their parameterized costs, i.e., learned cost models with updated feature values, except the partition count, down to the children operators. This is in contrast to the existing approach, where only a single cost (for a fixed pre-defined partition count) is computed for each physical operator. On reaching the stage boundary, the boundary operator explores the various partition values.
The second phase of {\it partition selection} starts with the boundary operator selecting the partition count that results in the optimal cost for all the operators in that stage. All operators in the stage then set the partition count as selected by the boundary operator in a bottom-up fashion, and then use it for estimating their learned cost.
This two-step approach avoids making local resource decision for each operator that may not be the best for the entire stage and even end up introducing additional stage boundaries.
Figure~\ref{fig:resourceopt}(d) illustrates the resource-aware planning approach for the running example. The planner explores $16$, $32$, and $64$ partitions for the first stage and finally picks $32$ partitions for the entire stage. Likewise, for the second stage, the planner explores $2$, $8$, and $16$ partitions and finally picks $16$ as the best partition count for that stage. 
%Algorithm~\ref{label:twophasealgo} shows the pseudo-code for the resource-aware query planner.

So far we described a two-phase query planning algorithm to incorporate resources in query planning and optimize for both the plan and the resources. 
The challenge, however, is that the resource exploration can explode the search space. 
Below we present techniques for efficiently navigating the resource search space.


\eat{
For making query planning resource-aware, we modified the optimize input phase top-down query optimization with the following two-phase approach, consisting of a 
partition exploration and a partition selection. 
Figures xx depicts the two phases.

In the partition exploration phase, each physical operator computes a vector of costs for a number of partition counts. This is in contrast to the existing approach, where only a single cost (for a pre-defined partition count) is computed for each physical operator. Since, exploring all partition counts is a fairly impossible goal, we choose a few partition counts for exploring the cost. 
}


\subsection{Efficient Resource Exploration }
\label{sec:eff_resource_exp}

%\new{added example to show how the space grows}
Big data systems can easily end up with a number of resource knobs to pick. For example, in a container based environment, the system already needs to pick the number of containers,  the memory size, and the cores in each container. The cloud environments can further expand the search space to the VM instance types, and other infrastructure level decisions. Exploring these resource choices at every single point in a query plan can grow the search space exponentially and make the resource-aware query planning infeasible. 
%More specifically, for estimating the cost of $m$ physical operators over
%$k$ resources, each with $n_1, n_2, n_3, ..., n_k$ possibles configurations, we need to explore $(n_1 * n_2 * n_3 * ... n_k)^m$ points in the optimal case. For instance, if we only consider using up to $100$ containers for $20$ physical operators, then we have a search space of $100^{20}$ points, clearly an infeasible tasks in existing optimizers.
Therefore, below we discuss two approaches for efficient exploration of resources, focusing only the partition count.

\eat{
\begin{algorithm}
	\vspace{-1pt}
    \scriptsize
	\Fn{OptimizeInput::Perform ()}{
	 	PhyOp $\leftarrow$ GroupExpr.GetPhyOp() \;
	 	\textcolor{blue}{
		StageLearnedModels $\leftarrow$ GroupContxt.GetStageLearnedModels() \;
		LocalLearnedModels	$\leftarrow$ GetLearnedModels(PhyOp) \;
		UpdateResourceAgnosticFeatureValues(LocalLearnedModels)\; 
		StageLearnedModels.AddLocalLearnedModels(PhyOp, LocalLearnedModels)\;	
		\If{PhyOp.IsBoundaryOpt()}{
			StageOptimalResource $\leftarrow$ FindOptimalResource(StageLearnedModels) (Sec 5.3)\;
			PhyOp.SetPartitionCount(StageOptimalResource.PartitionCount)\;
			StageLearnedModels.Clear()\;
		}		
		}
		\ForEach{ChildGroup $in$ GroupExpr.ChildrenGroups()}{
			\textcolor{blue}{
			ChildGroupContxt $\leftarrow$ 	ChildGroup.GetContext() \;
			ChildGroupContxt.SetStageLearnedModels(StageLearnedModels) \; 
			}
			OptimizeGroup(ChildGroup) \;
		}
		GroupExpr.ReDeriveProperties() \;
		ChildrenCost $\leftarrow$ PhyOp.GetChildrenCost()\;
		\textcolor{blue}{
		LocalCost $\leftarrow$ LocalLearnedModels.GetLearnedCost()\;
		}
		PhyOp.SetTotalCost(LocalCost, ChildrenCost)\;  
		} 
	\caption{Resource-aware query planning (we highlight the new additions in blue)}
	\label{label:twophasealgo}
\end{algorithm}
}



\eat{
\begin{algorithm}[t]
	\vspace{-1pt}
	\Fn{OptimizeInput::Perform ()}{
		PhyOp $\leftarrow$ GroupExpr.GetPhyOp() \\
		StageLearnedModels $\leftarrow$ OptContext.GetStageLearnedModels() \\
		LearnedModels	$\leftarrow$ LoadLearnedModels(PhyOp) \\
		OptContext.AddStageLearnedModel(PhyOp,LearnedModels); \\

		\If{PhyOp.IsBoundaryOpt()}{
			StageOptimalResource $\leftarrow$ FindStageOptimalResource(StageLearnedModels);			
			PhyOp.SetPartitionCount( StageOptimalResource.PartitionCount);
			StageLearnedModels.Clear()
		}
	
		\ForEach{ChildGroup $in$ GroupExpr.ChildrenGroups()}{
			ChildGroupOptContext $\leftarrow$ 	ChildGroup.GetOptContext() \\
			ChildGroupOptContext.SetStageLearnedModel( StageLearnedModels) \\
			OptimizeGroup(ChildGroup)
		}
		GroupExpr.ReDeriveProperties()\\
		ChildrenCost $\leftarrow$ PhyOp.GetChildrenCost()\;
		LocalCost $\leftarrow$ LearnedModels.GetLearnedCost()\;
		PhyOp.SetTotalCost(LocalCost,ChildrenCost)\;
	}
	\caption{TwoPhaseQueryPlanning}
	\label{label:twophasealgo}
\end{algorithm}
}



\subsubsection{Sampling-based Approach}

Instead of considering every single resource point, we could consider only a sample of them which result in significantly different costs. For partition counts, we could consider the values that are distributed uniformly over the entire range, i.e., from $1$ to the maximum number of containers available for the tenant or available in the cluster in case of single tenant. However, we notice that change in partition count has noticeable influence on cost when the value is small (e.g., 1 to 2), compared to when the partition count is already large (e.g., 1200 to 1250). Therefore, we sample the partition counts in a geometrically increasing sequence
 as follows: $x_{i+1} = \ceil*{x_{i} +x_{i}/s}$ with $x_0=1$, $x_1=2$, and $x_{i+1} < $ $P_{max}$, where $s$ is a skipping coefficient deciding how wide the gap is between successive samples. A large $s$ leads to large number of sample trials and thus more accurate predictions. However, this increases the prediction time. We found that $s=2$ is sufficient for most of practical purposes. As an example, for a maximum partition count of $3000$, we calculate local costs of operators for about $20$ partition counts.
We invoke learned cost models for each of the sampled partition counts to compute local costs. The set of local costs and their corresponding partitions are then passed down to the child operators. On reaching a boundary operator, we run the partition selection, i.e., the boundary operator selects the partition count that gives the optimal cost for all the operators in that stage. 
%\todo{add mathematical expression}
%For example, .... 
After boundary operator selects the stage optimal partition count, the rest of the operators set their partition count to the selected one, and then recompute the local learned costs.

Sampling based resource exploration bounds the search space when jointly exploring the optimal cost and partition counts.
However, there are two limitations of this approach:
(i)~low sampling frequency can result partition counts that are far from optimal, and
(ii)~high sampling frequency can quickly grow the number of model invocations, first for the individual learned models, and then for the combined model. 
Therefore, below, we discuss finding a single optimal partition count analytically using the operator model.

\subsubsection{Analytical Approach}

Instead of using all individual models as well as the combined model for exploring partition counts, we consider the relationship between the cost of the operator and the partition counts.
%
% using the Physical Operator, and follow an approach used by existing cost optimizers --- we first select the optimal partition count and then use it as a feature within the learned cost models. There are, however, key differences with the existing approach. First, we find the partition count that is optimal for the stage rather than only for the boundary operator. Second, we use a  learned model, derived out of the physical operator learned model, for selecting the partition count, rather than heuristics.
One option is to learn a separate resource model that captures the change in operator's cost as we vary the partition counts. However, we notice that we can reuse the learned operator model to derive the dependency on partition counts as follows: the dependency between the cost of an operator and the partition count is captured using the features where the partition count is involved. For instance, considering only the features related to partitions in operator learned cost model, we see that:

\vspace{0.1cm}
$cost \propto \frac{(\theta_1*I+\theta_2*C + \theta_3*I*C)}{P} + \theta_c*P$
\vspace{0.1cm}

\noindent During query optimization, we know $I$, $C$, $I*C$, therefore:

\vspace{0.1cm}
$cost \propto \frac{\theta_P}{P} + \theta_c*P$
\vspace{0.1cm}

%$\theta_P$ must be positive since cost of an operator should increase with the increase in $InputCard$ or $OutputCard$. 
\noindent Intuitively,  $\frac{\theta_P}{P}$ corresponds to the processing cost per partition, and $\theta_c*P$ corresponds to the overhead with each partition.
 The cost decreases with the increase in the partition count (due to less processing per partition) but after a certain number of partitions communication overhead dominates due to which the cost increases. Extending the above relationship across all operators on a stage, the relationship can be modeled as:

\vspace{0.1cm}
$cost \propto \frac{(\theta_{P1}+\theta_{P2}+...\theta_{Pn)}}{P} + (\theta_{C1}+\theta_{C2}+...\theta_{Cn})*P$
\vspace{0.1cm}

\noindent If only $(\theta_{C1}+\theta_{C2}+...\theta_{Cn})$ is negative,  there is no overhead of increasing the number of partitions and therefore we can have maximum number of partitions for the stage. 
Similarly, when only $\theta_{P1}+\theta_{P2}+...\theta_{Pn}$ is negative, we set the partition count to minimum as  increasing the partition count increases the cost. When both are either positive or negative, by differentiating the above equation with respect to P, we can derive the optimal partition count for the stage as follows:

\vspace{0.1cm}
$ P_{opt} = \sqrt{\frac{(\theta_{P1}+\theta_{P2}+...\theta_{Pn)}}{(\theta_{C1}+\theta_{C2}+...\theta_{Cn})}}$
\vspace{0.1cm}

\noindent Thus, during partition exploration, each operator calculates $\theta_{P}$ and $\theta_{C}$ locally, and passes them to the children operator. During partition selection, the boundary operator computes the optimal partition for the stage using the above formulation, thereby avoiding expensive resource exploration with multiple invocation of the learned cost models.

\subsection{Analysis}

Let us now analyze the effectiveness of the resource exploration techniques described above.
Consider a stage consisting of $n$ logical operators, with each logical operator having $m$ possible physical operator mappings. Let $P_{max}$ be the maximum possible partition count that a physical operator can be assigned. 
The naive approach is to consider every resource point and pick one partition count per stage.
At each resource point, we estimate the cost using four individual models, followed by the combined model.
%estimate the cost using the four models. 
Naturally, this results in $5\cdot m^n \cdot P_{max}$ cost model invocations.
For the sample-based approach, since we sample partition count in a geometric series sequence, with each successive sample being $(s+1)/s$ times the previous sample, we need to consider $log_{(s+1)/s}P_{max}$ samples for each physical operator. 
Each sample incurs five model invocations.
%For each sample, we first estimate the cost using four individual models, followed by the combined model. 
Thus, for each physical operator we need to make $5\cdot log_{(s+1)/s}P_{max}$ cost model invocations and for each stage we make $5m^nlog_{(s+1)/s}P_{max}$ invocations in the worst case. 
On the other hand, if we follow the analytical approach, we invoke the costs models for only one partition count and thus, overall, we make $5m^n$ models invocations, a factor $log_{(s+1)/s}P_{max}$ less than the sampling based approach.

To illustrate, consider the query shown in Figure~\ref{fig:resourceopt}, consisting of $8$ physical operators over $2$ stages. For a maximum of $3000$ partitions, it's clear that we need to make $120{,}000$ invocations using the naive approach, $800$ invocations using the sample-based approach, while only $40$ invocations using the analytical approach. 
Figure~\ref{fig:model_invocations} shows the number of model invocations with varying number of physical operators.
The analytical model incurs only few tens of invocations while the sampling-based approach can incur several thousands depending on the skipping coefficients.
In section~\ref{sec:experiments}, we empirically compare the accuracy of sampling strategy with different sample sizes with the analytical model, as well as with other sampling strategies such as uniform and random sampling.
%\todo{Highlight somewhere that sample based is still good if we want more accuracy; while analytical is good for lower overhead}






\begin{figure}
	\centerline {
		\hbox{\resizebox{\columnwidth}{!}{\includegraphics{figs/modelinvocations.pdf}}}}
	\vspace{-2.5pt}
	\caption{Model invocations for different sampling rates}
	\vspace{-0.5cm}
	\label{fig:model_invocations}
\end{figure} 

==> staging.tex <==
%!TEX root = main.tex

\section{Optimizer Integration}
\label{sec:integration}
\tar{Maybe, we will add a couple of paras on overall integration overview before talking about integration.}


For effectively integrating learned cost models with the optimizer, we need to solve two key challenges.

First, existing optimizers ignore the inter-operator parallelism between the pipelined operators during query optimization.
Instead, the overall cost is calculated as the sum of the cost of individual operators.
%, and corrected after the optimization to take into account the inter-operator parallelism. 
We discuss how we consider inter-operator parallelism during the optimization process itself in Section ~\ref{sec:interopt}.

Second, from Section 3.3, we know that the partition count of an operator impact its cost.
Moreover, earlier work \tar{cite ICDE paper, and maybe we need to add our own empirical results as well} suggest that costs of two physical operators can conflict depending on the machines (same as the number of partition counts) allocated to each operator.

Despite this fact, query optimization frameworks typically assume a fixed partition count (either a constant, or based on simple heuristics) during plan evaluation, which can result in sub-optimal plans. We discuss in Section~\ref{sec:resourceopt} how we make query optimization more partition-count-aware.

Finally, we present an algorithm in ~\ref{sec:algo} that considers both inter-operator parallelism  as well as optimal partition counts for the physical operators during query optimization.

We first outline two constraints from the query optimization framework that restrict our search 
space for addressing the two challenges.

\subsection{Optimizer Constraints}
\label{sec:constraints}

\tar{Maybe better to highlight these things in the Background section, writing it here for now to make the reasoning behind some of the decisions in the later sections clear.}

Query optimizer frameworks follow either a top-down or bottom-up query evaluation approach, which puts restrictions on the s\\
pace of plans we can search during query optimization. 
Scope is based on Cascade Framework, which is a top-down query optimization framework.  
In Cascade, physical operators are selected bottom-up in a query plan, with the following two constraints:
\begin{enumerate}[noitemsep,parsep=0pt,partopsep=0pt,leftmargin=*]
\item  We do not know the physical operators of the parent nodes until we have already selected the physical operators of the children nodes.
\item Physical operators once selected for the bottom nodes cannot be changed.
\end{enumerate}

However, we are allowed to traverse the query plan down, and change the properties or estimated cost of an operator, given they do not invalidate the part of the query plan already selected. We leverage this technique in our algorithm in Section~\ref{sec:algo}. \tar{need to double check this with Shi.}


\subsection{Inter-Operator Parallelism Awareness \aj{clarify!}}
\label{sec:interopt}

We first explain the modeling that considers inter-operator parallelism, and then discuss how we use the model during query optimization.

\subsubsection{Modeling}

We, first, define a few terms that we will use in the cost modeling. 

A physical query plan, $plan$, can broken down as a sequence of multiple fragments $frag_1, frag_2, ..., frag_n$, where a fragment is defined as follows.
\begin{definition}[fragment]
 Fragment is a sub-graph between two blocking operators (e.g., sort, aggregate),  including the top blocking operator. All operators within the same fragment execute concurrently, except the top blocking operator, which doesn't starts its execution  until it has received all input tuples. A stand-alone blocking operator (with another blocking operator as a children) is also a fragment.  \tar{Note that we are moving away from our earlier assumption that operators across stages cannot be pipelined --- I think exchange operators can be pipelined with other operators unless they are blocking. On the other hand, if we have a sort operator in a stage, it's blocking and therefore not pipelined with other operators on the same stage.}
\end{definition}

\begin{definition}[first-tuple cost]
First-tuple cost is the time taken by an operator to produce the first ouput tuple after receiving the first input tuple.
\end{definition}

\begin{definition}[processing cost]
Processing cost is the time taken by an operator to produce the rest of the ouput tuples after producing the first output tuple.
\end{definition}


Let $cf_i$ be the cost of a fragment $frag_i$, with $n$ pipelined-physical operators, $pl_1,pl_2, ...,pl_n$ and a blocking operator $pbl$. Let their first-tuple costs be: 
$f_1,  f_2, ..., f_n, f_{bl}$, and processing costs: $p_1,  p_2,\\  ..., p_n, p_{bl}$ . Then, the cost of a fragment, $cf_i$ (when $i \neq n$), except the topmost is defined as the time taken by the fragment from consuming the first input tuple to producing the output tuple: $cf_i = \sum_i f_i + max_i(p_i) + f_{bl} $

However, the cost of the last or topmost fragment is the time taken by the fragment  from consuming the first input tuple to producing the \emph{last} tuple: $cf_n = \sum_i f_i + max_i(p_i) + f_{bl} + p_{bl} $

The overall cost of the plan is thus: $cost_{plan} = \sum_i cf_i$

Next, we discuss how we modify the query optimizer to use this modeling during query evaluation.

\subsubsection{Integration with Optimizer}
\label{sec:interoptintegration}
Our goal is to make the optimizer inter-operator parallelism aware within the two constraints discussed in Section~\ref{sec:constraints}. Our key idea is that we look at the granularity of fragment instead of an operator. In particular, while evaluating a physical operator, earlier we used to calculate overall cost as a sum of operator's local cost and children operators' cost. Now, instead of using operator's local cost we use its fragment cost as the local cost. Similarly, for children cost, instead of looking at the children operators' cost, we consider children fragments' costs.
We state the algorithm more formally below.

\tar{a rough sketch, I will try to expand it a bit and formalize it more}

Let the physical operator selected be $po$ for a given logical operator, and assume that it belongs to fragment $frag$. Let the cost of the $frag$ be $cf_{po}$.
We identify the the input fragments to $frag$ by traversing down the tree until we reach the last pipelined operator in the fragment. Let the input fragments to $frag$ be $frag_{c1}$, $frag_{c2}$, $...$ and $frag_{cn}$. Let their costs be $cf_{c1}, cf_{c2}, ..., cf_{cn} $. The cost of the theses fragments are the costs of their root operators.

Now, children fragments cost for $po$ = $max(cf_{c1}, cf_{c2}, ..., cf_{cn})$.

Overall cost of the subgraph with root operator $po$, is thus = $cf_{po}$ + $max(cf_{c1}, cf_{c2}, ..., cf_{cn})$.

\subsection{Optimal Partition Count Selection}
\label{sec:resourceopt}
Here the goal is to select the optimal partition counts for each operator. There are two challenges to solve. 

First, how do we decide which partition counts to explore for a physical operator during query optimizations. Since, exploring all partition counts is a fairly impossible goal, we learn a model for each physical operator offline that we probe online for quickly identifying optimal partition counts. We describe how we learn this model in the next section.

%would need to explore all possible partition configurations for each candidate operator during query optimization, with an overall large search space, a goal that is fairly impossible to achieve.

%Therefore, we first learn a minimal set of optimal partition counts for each physical operator offline, and limit our exploration to pre-selected partition counts for each physical operator during query optimization.

Second, how do we modify the optimization framework to also explore partition counts of a physical operator. In other words, we need to extend the approach discussed in Section~\ref{sec:interoptintegration} to also consider different partition counts for a physical operator during plan evaluation. We discuss how we do it in Section~\ref{sec:algo}.

\subsubsection{Profiling Physical Operators}

Our goal is  model the runtimes of physical operators as a function of input partition size, output partition size, and the number of partitions. For this, we reuse the cost model that we learnt for a physical operator, considering all features other than those related with parition counts as a constant ($a$ below). More formally, 

\noindent
$L(op)$ = $a+b*I+c*O+d*{pc}$

\noindent
where,

\noindent
$I=\frac{InputCard*AvgRowLen}{pc}$  (input partition size)

\noindent
$O= \frac{OutputCard*AvgRowLen}{pc}$ (output partition size)


$b*I$ captures how the performance of a single machine varies with increase in input data size. $c*O$  captures how the performance of a single machine varies with increase in output data size. $d*pc$ captures communication overhead. As we increase the number of partition counts, processing cost per partition decreases. However, with the increase in number of partition, there is also an increase in communication overhead, which may increase L. 

Now, during query optimization, we will have all the parameters available from the query itself, except the partition count. So for finding the partition counts for minimum runtime, we differentiate the above equation with respect to $pc$ and set it to 0, selecting those $pc$ values that are minima.

%However, two operators in the same stage cannot have different parition counts.


\subsubsection{Integration with Optimizer}
\label{sec:algo}
We first state the problem setting.

Given a physical operator $po$ belonging to a fragment $frag$ and stage $st$, we want to find the partition count $x$ for $po$ such that the cost of the $frag$, $cf_x$, is minimum. 

Note that on setting the partition count of $po$ to $x$, we also need to set the partition count of all operators below $po$ in $st$, including the output partition of the exchange operator below it to $x$. For ease of explanation, we assume there is a single child operator of $po$, and that there is  no fragment below $frag$ in the stage $st$. Let the partition count of the child operator of $po$ be $x1$. 

Here is a rough sketch of the algorithm.

\begin{enumerate}[noitemsep,parsep=0pt,partopsep=0pt,leftmargin=*]

\item We first find out the fragment cost of $frag$ by setting the partition count of $po$ to be $x1$, the same partition count as that of the child operator. Let that be $cf_{x1}$

\item  We find out the partition count for which $po$ has a minimum local cost. Let that partition count be $x_2$.  (Ideally there could be more than one, for ease of explanation, let's assume there is only one).

\item If$x_2 \neq x_1$  we set the partition counts of all operators in $st$ (including $po$ and the output partition count of exchange operator below it) to $x_2$, and calculate the fragment cost. Let that be $cf_{x2}$. 
%(If there is another fragment below $frag$ in the same stage, we adjust their cost as well. We ignore that case for ease of explanation for now.)

\item If  $cf_{x1} <= cf_{x2}$, we set the partition count of $po$ to $x1$, and we are done. Otherwise, it means that optimal partition count for $po$ and operators below $po$ in $st$ conflict, and therefore we resolve it using the next step.

\item We probe multiple partition counts between $x_1$ and $x_2$ using binary search. For a given partition count say $y$, we follow a step similar to 3, we set the partition count of all the operators of the $st$ and the output partition count of exchange operator below it to $y$, and calculate the fragment cost. We also consider a case where we add an exchange operator just below $po$. Finally we select $y$ for which the $frag$ has minimum cost.

\end{enumerate}

\eat{
\textbf{Key Insight.} Note that the cost of stage is dominated by the physical operator taking the maximum time, so we incrementally change the resources of that operators to bring the cost of overall stage down.


Unfortunately, we found that exploring even a few optimal resource configurations within the existing optimization frameworks is an extremely hard problem, and requires a new query optimization framework for joint optimization of queries and resources. We, instead, use a simple approach that is good \tar{fix}. We discuss the second stage in more detail in Section~\ref{resourc-staging-intg}. 

We evaluate the partition counts at the granularity of stage, i.e, on reaching the exchange operator, we try to adjust the partition counts of the operators belonging to stage below the exchange operator such that overall cost of the stage is optimal.
In other words, we first select the the physical operators within the stage using the default partition count selected by the existing cost models, and then try to improve the cost of the fragment by modifying the partition counts of the operators in the stage.

We do it at the granularity of stages for several reasons:
1) optimal partition count for one operator can be sub-optimal for other operator; 2) if the operator is non-blocking, we cannot be sure if it's cost will 
contribute the overall cost, 3) combined exploration space of physical operators and partition counts together is large.

Now we state the problem:
\begin{problem}
Given a stage, consisting of physical operators, find partition counts for each of the operators in the fragment such that the overall cost for the fragment is minimum.
\end{problem}

Note recall that changing the partition count for an operator inside the fragment can lead to addition of an exchange operator in the fragment. We propose two algorithms:

\smallskip
\noindent
\textbf{DP-based branch and bound algorithm.} Here we try to explore the space of PPIs profiled offline for each operator in the fragment. If the PPI of two consecutive operator is distinct, we add an exchange operator and add it's cost as well.

\smallskip
\noindent
\textbf{Greedy algorithm.} Here we exploit the fact that the cost of fragment is the max of the individual costs of the operators, and moreover we know that we want to minimize the number of exchange operators.
}






\subsection{Feedback Infrastruture}
-- learned model feedback

-- multi-model for the same logical subgraph

-- applying learned model

-- model testing: ability to predict and pass values offline

-- Briefly remind about the other two challenges we introduced in Section 2:
Resource optimization, Staging-awareness.


